Online Algorithms for the Santa Claus Problem

The Santa Claus problem is a fundamental problem in fair division: the goal is to partition a set of heterogeneous items among heterogeneous agents so as to maximize the minimum value of items received by any agent. In this paper, we study the online version of this problem where the items are not known in advance and have to be assigned to agents as they arrive over time. If the arrival order of items is arbitrary, then no good assignment rule exists in the worst case. However, we show that, if the arrival order is random, then for $n$ agents and any $\varepsilon > 0$, we can obtain a competitive ratio of $1-\varepsilon$ when the optimal assignment gives value at least $\Omega(\log n / \varepsilon^2)$ to every agent (assuming each item has at most unit value). We also show that this result is almost tight: namely, if the optimal solution has value at most $C \ln n / \varepsilon$ for some constant $C$, then there is no $(1-\varepsilon)$-competitive algorithm even for random arrival order.

==> TrashFiles/dec28_notes.tex <==
\begin{document}
\section{Lower bound notes}
We want to reformulate our ``public" and ``private" good example with the intuition of Agrawal's optimal lowerbound of $\Omega(\log n / \varepsilon^2)$. The idea is the following:
\vspace{2.5mm} \\
Let $s_i = \text{Binom}(B, p)$ be the distribution which gives us a 1 if an item is private to agent $i$ and public otherwise (i.e. $B - s_i$ public items contributed by agent $i$). The public items are where any algorithm has the potential to make (constant probability) mistake in assignment.
\vspace{2.5mm} \\
Let $\{s_1, ..., s_n\}$ denote the set of private items to agents $i \in [n]$ and $s_{\min} = \min_i \{s_1, ..., s_n\}$. Note that in the definition of these iid Bernoulli distributions, we want $p$ to be large enough such that for any $\varepsilon > 0$ we have $$\varepsilon B \approx B - s_{\min} \Rightarrow s_{\min} \approx (1-\varepsilon)B$$
\vspace{2.5mm} \\
In expectation, what is the value of $s_{\min}$? Using the normal approximation of a Binomial distribution, $\mathcal{N}(Bp, Bp(1-p))$ we can directly compute the expectation using $$\mathbb{P}(\min_i s_i \leq t) = 1 - \left[1-F(t)\right]^n$$
\subsubsection{Gautam Class Notes}
Above resource gives us that for $Y = \max_i \{X_1, ..., X_n\}$ where $X_i ~ \mathcal{N}(0, \sigma^2)$ are iid, then we have the bounds $$\frac{1}{\sqrt{\pi \log 2}} \sigma \sqrt{\log n} \leq \mathbb{E}[Y] \leq \sqrt{2}\sigma \sqrt{\log n}$$ which we can extend using the Normal approximation for Binomials to get an upper bound of $O(\log^{1/2} n)$ on the \emph{maximum}.
\vspace{2.5mm} \\
Alternatively, we can directly compute the expectation of $Y = \min_i s_i$ as $$\mathbb{E}[Y] = p^{Bn} \sum_{t=1}^B \left( \sum_{j=t}^B \binom{B}{j} \right)^n$$ For large $n$ this behaves like $$(1-p^{B})^{n}$$

\end{document}

==> TrashFiles/dec8_notes.tex <==
\begin{document}
\raggedbottom
\section{Problem Defintion and Preliminaries}
We seek to allocate a set of $m$ indivisible goods ($\mathcal{M} = [m]$) equitably across $n$ agents ($\mathcal{N} = [n]$), where $n \leq m$. In particular, we define a \emph{fair allocation} as one that maximizes the minimal bundle value to any agent (the so-called \textsc{MaxMin} problem). Formally, let $v_{ij}$ denote the value of good $j$ to agent $i$ and let $\mathcal{S}_i$ denote the subset of items allocated to agent $i$. The problem described above is thus $$\max \min_i \sum_{j \in \mathcal{S}_i} v_{ij}$$ and can be formulated with the following LP relaxation
\begin{gather*}
\max \lambda \\
\begin{aligned}
\textup{s.t.}\quad &\forall i \in \mathcal{N} \quad \sum_{j \in \mathcal{S}_i} v_{ij} \cdot x_{ij}  \geq  \lambda \\
            &\forall j \in \mathcal{M} \quad \sum_i x_{ij} \leq 1
\end{aligned}
\end{gather*}
where $x_{ij}$ denotes the fraction of item $j$ assigned to agent $i$. In this work, we further reduce the problem to that of the \emph{Santa Claus problem} with unit valued goods: $v_{ij} \in \{0,1\}$ for all $j \in \mathcal{M}$.

We examine the \textsc{MaxMin} problem from the online setting, where goods to be allocated arrive one at a time and need to be permanently assigned to an agent upon arrival. We will examine this problem under both the IID, random-order and adversarial frameworks. We assess the quality of our algorithms by their \emph{competitive ratio}, or the ratio of our online algorithm's solution to that of the optimal \emph{offline} solution (denoted \opt{}). More formally, let $\mathcal{I}$ denote an arbitrary problem instance and \textsc{Alg} denote the solution value output by the designed online algorithm, then the competitive ratio is at least $c$ when, for constant $b \geq 0$: $$\textsc{alg}(\mathcal{I}) \geq c \cdot \opt{}(\mathcal{I}) - b$$

\section{Adversarial Counterexamples}
We here present lower bounds on the problem context under an adversarial input model. This is the setting in which an adversary presents a worst-case input by selecting both the item values for each agent and the order in which items arrive (thus constructing the difficult allocation problem istances). Our first result of this kind is the following theorem.

\begin{theorem} \label{thm.determin_bound}
    The competitive ratio of any deterministic algorithm is zero under the adversarial arrival input model.
\end{theorem}
\begin{proof}
    Let \textsc{alg} be a fixed deterministic algorithm and assume that the adversary picks the first item to have value 1 for all $n$ agents. Assume \textsc{alg} allocates this item to the first agent without loss of generality. Now for the following $n-1$ items, the adversary presents items of value 1 to all agents but the $n$-th agent. Then regardless of how \textsc{alg} assigns these items, $v_n(\mathcal{S}_n) = 0$ whereas the optimal offline allocation would have given the first item to this agent (\opt{} $= 1$). Thus, the competitive ratio is 0.
\end{proof}

\begin{theorem} \label{thm.simple_counter}
    There is no randomized algorithm that obtains a competitive ratio better than $\frac{1}{n}$ for the online \textsc{MaxMin} problem in the adversarial input model.
\end{theorem}
\begin{proof}
    \todo{add proof, similar to above counterexample and invoke Yao's principle.}
\end{proof}

\begin{theorem}
    For any algorithm for the online \textsc{MaxMin} problem in the random order model, there exists an instance such that its competitive ratio is less than $1 - \Omega(\varepsilon)$ when $$\opt{} \geq \frac{\log n}{\varepsilon^2}$$ Or, equivalently, no algorithm can achieve a competitive ratio better than $1-\Omega(\sqrt{\log n / \opt{}})$.
\end{theorem}
\begin{proof}
    We prove this by constructing an allocation instance with $nk$ items, where $n$ is the number of agents in the system and the optimal offline solution ($\opt{}$) is $k$ such that no online algorithm can achieve a competitive ratio of $1-O(\varepsilon)$ unless $\opt{} \geq (\log n / \varepsilon^2)$.
    
    In this construction, we define $n+1$ item types. The first type has a value of $1$ to all $n$ agents, which we call a ``public" item, and the remaining $n$ types have value $1$ to exactly one agent (i.e. $v_{ij} = 1 \iff i=j$) which we call ``private" to agent $i$. We will construct $k$ items for each agent, which have an equal probability of being private to said agent or public. Thus, our constructed instance consists of
    \begin{itemize}
        \item $s_i$ inputs for each agent $i$ which is private to that agent, where $s_i$ is a random variable following binomial($k,1/2$).
        \item $k-s_i$ inputs for each agent $i$ which are public to all agents.
    \end{itemize}
    
\end{proof}

\begin{theorem} \label{thm.opt_lower}
A randomized algorithm can achieve a nonzero competitive ratio if and only if the optimal offline solution is at least $\log n$. \todo{Restate, this is not the proper framing of the result.} % This algorithm should refer to the additive log factor, mot competitive ratio. If we 
\end{theorem}
\begin{proof}
    Assume we have $n$ agents and $n$ item \emph{types} which are broken down in the following way: items $n_i$ for $i \in [n-1]$ are ``private" meaning they have value 1 to their corresponding agent $i$ and 0 for the others ($j \neq i$). Lastly, the $n$-th item type is ``public" meaning it has a value of 1 for all agents. Further assume we have $k$ of each item type, giving us $nk$ total items. 
    
    In the offline scenario, each agent receives exactly $k$ items of their specific type (where the agent without a private good must receive all the public goods) to achieve $\textsc{opt} = k$. Analysis of the error in our online setting is measured in terms of how many of the public goods are assigned \emph{improperly}, since the private goods will always be correctly assigned (as they can only be allocated to their corresponding agent). As such, we have that public goods can be assigned improperly until the identity of all agents as either public or private is revealed. Therefore, we examine $N$: the number of iterations it takes to see at least one of each item type.
    
    For each $i \in [n]$, define $A_{i,m}$ to be the event that we \emph{do not} see item type $i$ in the first $m$ iterations. We thus have for $1 \leq j \leq n$
    $$P(A_{1,m} \cap A_{2,m} \cap \dots \cap A_{j,m}) = \binom{(n-j)k}{m} \Big/ \binom{nk}{m}$$
    Now define $B_m$ to the be the event that some item type has not been sampled after $m$ draws, we combine the above result with the Principle of Inclusion Exclusion \cite{} to find
    $$P(B_m) = \sum_{j=1}^n (-1)^{j-1} \binom{n}{j} \binom{(n-j)k}{m} \Big/ \binom{nk}{m}$$
    We can now derive the expected value of $N$ by utilizing the results above in the following manner:
    \begin{align*}
        \mathbb{E}[N] &= \sum_{m=0}^\infty P(N > m) = \sum_{m=0}^{nk} P(B_m) \\
        &= \sum_{m=0}^{nk}\sum_{j=1}^n (-1)^{j-1}\binom{n}{j} \binom{(n-j)k}{m} \Big/ \binom{nk}{m}
    \end{align*}
    We now directly compute the constituents of this sum by using the beta function of each binomial coefficient:
    \begin{align*}
        \mathbb{E}[N] &= \sum_{m=0}^{nk}\sum_{j=1}^n (-1)^{j-1}\binom{n}{j} \binom{(n-j)k}{m} \Big/ \binom{nk}{m} \\
        &= (nk+1)\sum_{m=0}^{nk}\sum_{j=1}^n (-1)^{j-1}\binom{n}{j} \binom{(n-j)k}{m}\int_0^1 x^m (1-x)^{nk-m} dx
    \end{align*} % Had to split apart for now but hopefully can fit on one page when other stuff is added.
    \begin{align*}
        &= (nk+1) \sum_{j=1}^n (-1)^{j-1} \binom{n}{j} \int_0^1 (1-x)^{jk} (x+(1-x))^{(n-j)k}dx \\
        &= (nk+1) \sum_{j=1}^n (-1)^{j-1} \binom{n}{j} \int_0^1 (1-x)^{jk} dx \\
        &= (nk+1) \sum_{j=1}^n (-1)^{j-1} \binom{n}{j} \int_0^1 t^{jk} \tag*{($t = 1-x$)}\\
        &= (nk+1) \int_0^1 (1 - (1-t^k)^n) dt \\
        &= (nk+1) \left(1 - \frac{1}{k} \int_0^1 (1-s)^n s^{1/k - 1} ds \right) \tag*{($s = t^k$)}\\
        &= (nk+1)\left( 1 - \frac{\Gamma(n+1)\Gamma(1/k)}{k\Gamma(n+1/k+1)} \right) \\
        &= (nk+1)\left(1 - \frac{n!}{(1+1/k) \cdot (2 + 1/k) \cdot  \dots \cdot (n+1/k)} \right) \\
        &= (nk+1)\left( 1 - \frac{e^{O(1/k)}}{(n+1)^{1/k}} \right) \tag*{(Stirling approx.)}\\
        &= (nk+1)\left( 1 - \exp{\frac{-\log n + O(1)}{k}}\right) 
    \end{align*}
    We now consider two distinct cases for the parameter $k$.
    \vspace{2.5mm} \\
    \underline{\textit{Case I.}} $k  \ll \log n$ \\
    For the assumption on $k$, we have that $\exp{\frac{-\log n + O(1)}{k}} \approx 0$. Therefore, we can approximate the expectation by $$\mathbb{E}[N] \approx nk$$
    \underline{\textit{Case II.}} $k \gg \log n$ \\
    We see that when $\lim_{n \rightarrow \infty} \log n / k = 0$ we have that $\frac{\log n + O(1)}{k}$ is small so we can make the Taylor approximation
    $$\mathbb{E}[N] \approx (nk+1) \left( \frac{\log n + O(1)}{k} \right) = n \log n + \frac{O(1)}{k} \approx n \log n$$
    \todo{Relate back to competitive ratio.} \\
    Therefore, when $k$ is constant, in expectation we will sample the entire set before realizing the public agents identity. Thus, we require that $\textsc{opt} = k \gg \log n$ in order to achieve a nonzero competitive ratio for the online algorithm.
\end{proof}

\section{IID Model}
Let \opt{} denote the maximal value achieved in the offline setting to the \textsc{MaxMin} problem. We will here assume that the value of \opt{} is known (or can be estimated with minimal reduction in approximate value). Our algorithm works by greedily assigning items according to an exponential reward function. We define the following potential function $$\phi(k) = \left(\frac{\alpha \ln n}{\opt{}}\right) \exp \left(- \frac{\alpha \ln n}{\opt{}} \cdot k \right)$$ where the value of $\alpha$ is to be defined later. We additionally define $$\overline{\Phi}(k) = \int_{s=k}^{\infty} \phi(s) ds$$
We can thus define the ``remaining reward" for agent $i$ at any stage of the algorithm by $\overline{\Phi}_i = \overline{\Phi}(c_i)$ where $c_i$ is the current coverage of agent $i$, and the \emph{overall} remaining reward is $\overline{\bold{\Phi}} = \sum_{i \in \mathcal{N}} \overline{\Phi}_i$.
\vspace{2.5mm}\\
Let $j$ be the current request in the input stream. If the fractional coverage is $c_i$ for some agent $i$, then the reward $r_{ij}$ of allocating $j$ to $i$ is the \emph{decrease} in the value of $\overline{\bold{\Phi}}$: $$r_{ij} = \int_{s=c_i}^{c_i + v_{ij}} \phi(s) ds$$ The \textsc{MaxMin} algorithm greedily assigns impressions based on this reward function. We now derive the competitive ratio of the above greedy approach where we assume the item values are drawn from an unknown IID distribution. 
\begin{theorem} \label{thm.reward_comp}
    For any $\varepsilon > 0$, the competitive ratio of the above algorithm for the \textsc{MaxMin} problem is $1-\varepsilon$, assuming $\opt{} > \frac{\log n}{\varepsilon}$.
\end{theorem}
\noindent  We first make the definition $\opt{} = \alpha \ln n$ where $\alpha > \frac{1}{2\varepsilon}$ in accordance with the assumption on \opt{} (and the result of Theorem \ref{thm.opt_lower}). In proving the theorem, we first assemble useful results which will combine to yield the proof.
\begin{lemma} \label{lemma.LPbound}
    At any stage of the algorithm, the expected decrease in $\overline{\bold{\Phi}}$ for the next arriving impression is at least $(1-\varepsilon)\frac{\alpha \ln n}{m}\overline{\bold{\Phi}}$.
\end{lemma}
\begin{proof}
    In proving this lemma, we examine the expected LP formulation of the problem. We compare the decrease in potential of our algorithm to that of the hypothetical (fractional) algorithm which exactly follows the LP assignment. We note that this LP is used only for analysis, as the algorithm cannot use it since it does not know the distribution from which the input is sampled. Our algorithm maximizes the decrease in potential at every step, and therefore any lower bound on the expected decrease in the LP-based algorithm is \emph{also a lower bound for our algorithm} by optimality of the solution. We reiterate that our algorithm yields an integral solution and cannot use the above LP.
\begin{gather*}
\begin{aligned}
    \sum_{\xi} p(\xi) \cdot v_{i}(\xi) \cdot x_{i}(\xi)  \geq  \frac{\lambda}{m} \quad &\forall i \in \mathcal{N} \\
    \sum_i x_i(\xi) = 1 \quad &\forall i \in \mathcal{N}, \xi\\
    0 \leq x_{i}(\xi) \leq 1 \quad &\forall j \in \mathcal{M}, \xi
\end{aligned}
\end{gather*}
In the LP, $\xi$ indexes the support of the distribution from which impressions are sampled, $p(\xi)$ denotes the probability of any impression having type $\xi$, and as before $x_i(\xi)$ denotes the fractional allocation to agent $i$. The first constraint ensures that each agent is assigned at least the optimal amount in expectation and the second ensures that impressions are allocated in their entirety. The expected decrease in $\overline{\bold{\Phi}}$ for an algorithm which fractionally assigns impression $j$ with probability $x_i(\xi)$ at any stage is 
\begin{gather*}
    \sum_i \sum_{\xi} p(\xi) \cdot x_i(\xi) \int_{k=c_i}^{c_i + v_i(\xi)} \phi(k) dk \\
    = \sum_i \sum_{\xi} p(\xi) \cdot x_i(\xi) \cdot \phi(c_i) \cdot v_i(\xi) \cdot \left( \frac{\opt{}}{\alpha v_i(\xi) \ln n} \right)\left(1 - e^{\frac{- \alpha v_i(\xi) \ln n}{\opt{}}}\right)
\end{gather*}
Using the fact that $\frac{1-e^{-x}}{x} \geq 1 - \frac{x}{2}$ from Taylor expansion, we thus obtain
\begin{gather}
    \geq \sum_i \sum_{\xi} p(\xi) \cdot x_i(\xi) \cdot \phi(c_i) \cdot v_i(\xi) \cdot \left( 1 - \frac{\alpha v_i(\xi) \ln n}{2 \opt{}}\right) \\
    \geq \sum_i \sum_{\xi} p(\xi) \cdot x_i(\xi) \cdot \phi(c_i) \cdot v_i(\xi) \cdot (1-\varepsilon)
\end{gather}
where the second inequality comes from $v_i(\xi) \leq 1$ and the assumed bound on \opt{}. Finally, rearranging the terms and utilizing the first constraint from the expected LP gives us
\begin{gather*}
    \geq (1-\varepsilon) \sum_i \frac{\phi(c_i) \opt{}}{m} = (1-\varepsilon)\frac{\alpha \ln n}{m} \overline{\bold{\Phi}}
\end{gather*}
\end{proof}
\noindent We now prove the following corollary that demonstrates how Lemma \ref{lemma.LPbound} gives us the proof of Theorem \ref{thm.reward_comp}.
\begin{corollary}
    The expected value of $\overline{\bold{\Phi}}$ at the end of the algorithm is at most $n^{1-(1-\varepsilon)\alpha}$.
\end{corollary}
\begin{proof}
We denote the decrease in $\overline{\bold \Phi}$ by $\Delta\left( \overline{\bold \Phi}\right)$. The above lemma implies that $\mathbb{E}[\Delta\left( \overline{\bold \Phi}\right)] = (1-\varepsilon)\frac{\alpha \ln n}{m} \overline{\bold{\Phi}}$. Therefore, after each allocation, we have:
$$\overline{\bold \Phi} - \mathbb{E}\left[\Delta\left( \overline{\bold \Phi}\right)\right] = \left(1 - \left(1-\varepsilon\right) \frac{\alpha \ln n}{m} \right) \cdot \overline{\bold{\Phi}} \leq n^{-(1-\varepsilon)\frac{\alpha}{m}} \cdot \overline{\bold{\Phi}}$$
where the inequality invokes $1-x \leq e^{-x}$. By the linearity of expectations, when starting from a value $\overline{\bold{\Phi}}_0$, the expected value after $m$ impressions is given by
\begin{align*}
    \overline{\bold{\Phi}}_0 - \mathbb{E}\left[\Delta\left( \overline{\bold \Phi}_0\right) + \dots + \Delta\left( \overline{\bold \Phi}_m\right)\right] &\leq \overline{\bold{\Phi}}_0 - \mathbb{E}\left[m \Delta\left( \overline{\bold \Phi}_0\right)\right] \\
    &= \overline{\bold{\Phi}}_0 - m\mathbb{E}\left[\Delta\left( \overline{\bold \Phi}_0\right)\right] \\
    &= \left(1 - m \cdot \left(1-\varepsilon\right) \frac{\alpha \ln n}{m} \right) \cdot \overline{\bold{\Phi}}_0 \\
    &\leq n^{-(1-\varepsilon)\alpha} \overline{\bold{\Phi}}_0
\end{align*}
Lastly, noting that $$\overline{\bold{\Phi}}_0 = \sum_i \overline{\Phi}(0) = \sum_i 1 = n$$ we have that the expected value when the algorithm terminates is at most $n^{1-(1-\varepsilon)\alpha}$.
\end{proof}
\noindent We can now prove Theorem \ref{thm.reward_comp} by contradiction.
\begin{proof}
    Assume for some agent $i_{\min}$ that the fraction coverage $c_{i_{\min}} < (1-\varepsilon) \opt{}$ at the algorithms termination. Then,
    $$\overline{\bold{\Phi}} = \sum_i \overline{\Phi}_i \geq n \cdot \overline{\Phi}_{i_{\min}} = n \cdot n^{-\frac{c_{i_{\min}}}{\opt{}}} > n \cdot n^{-(1-\varepsilon)\alpha} = n^{1-(1-\varepsilon)\alpha}$$ which contradicts the expected maximal value of $\overline{\bold{\Phi}}$ at the end of the algorithm. Therefore, each $c_i \geq (1-\varepsilon) \opt{}$.
\end{proof}

\section{Random Order Model}
\todo{Adapt the expected LP for the random order model and get the identical result?}

\section{Notes}
\subsection{Additive loss factor / budget constraint lower bound (Agrawal paper)}
Essentially, they construct a rather complicated counterexample with an adversarial problem instance such that $$\opt{} < 7B$$ where $B$ is the budget parameter. They subsequently show that the algorithm output is upperbounded as $$\textsc{alg} \leq \opt{} - (P + M)$$ where the $P$ and $M$ are parameters / functions of other parameters for this counter. Thus in order to have $$\opt{} - (P + M) < \opt{} - \varepsilon \opt{}$$ whic is furthermore bounded above as $$7B - \varepsilon 7B{} = (1-\varepsilon)7B$$ we thus must have that $P + M < 7\varepsilon B$.
\vspace{2.5mm} \\
With respect to our counterexample, it seems we could phrase our $\log n$ expected loss proven above as $$\textsc{alg} \geq \opt{} - \Gamma$$ where $\Gamma = O(\log n)$ and thus to have a $1-\varepsilon$ competitive ratio we require $$\opt{} - \Gamma > \opt{} - \varepsilon \opt{} \Rightarrow \opt{} > \Gamma / \varepsilon = O(\frac{\log n}{\varepsilon})$$ but with the analysis being more careful?

\subsection{Random order model}

\end{document}

==> TrashFiles/dp-adversarial.tex <==
\subsection{Algorithm}

We show the following:

\begin{theorem}\label{thm:ad-lower}
    In the adversarial setting, for any $\e \in (0, 1)$, there is an algorithm for the online Santa Claus problem that has a competitive ratio of $(1-\e)\cdot\frac1n$ for $\opt > C\cdot \frac{n\ln n}{\e^2}$ for a large enough constant $C$.
\end{theorem}
\begin{proof}
    The algorithm is to simply assign every item uniformly at random among all the $n$ agents. Note that for any fixed agent, its expected value is at least $\frac1n \cdot \opt$. By Chernoff bounds, the probability that its total value is less than $(1-\frac\e2)\frac1n \cdot \opt$ is given by 
    $\exp(-\frac12\cdot \frac{\e^2}{4}\cdot \frac1n \cdot \opt) < \frac{\e}{2n}$ for $\opt > C\cdot \frac{n \ln n}{\e^2}$ for a sufficiently large constant $C$. By union bound over all the $n$ agents, the probability that {\em any} agent's overall value is less than $(1-\frac\e2)\frac1n\cdot\opt$ is at most $\frac\e2$. Thus, the expected competitive ratio is at least $(1-\frac\e2)(1-\frac\e2)\cdot \frac1n > (1-\e)\cdot \frac1n$.
\end{proof}

\subsection{Impossibility Result}

We show the following:

\begin{theorem}\label{thm:ad-upper}
    In the adversarial setting, no algorithm can obtain a competitive ratio better than $\frac1n$.
\end{theorem}
\begin{proof}
    We consider the following instance. Of the $n$ agents, $n-1$ are private agents each having $k$ private items that have valuation $1$ for the corresponding private agent and $0$ for every other agent. The $n$th agent is a public agent and there are $k$ public items that have a valuation of $1$ for all the $n$ agents. The optimal solution assigns the private items to the corresponding private agents and the public items to the public agent. Thus, $\opt = k$. In the online instance, the public items arrive before the private items. Since all the agents look identical before the arrival of the first private item, the public agent gets no more than $k/n$ items in expectation for any algorithm. The theorem follows.
\end{proof}

==> TrashFiles/dp-lower.tex <==
\newcommand{\alg}{\textsc{\sc alg}\xspace}
\renewcommand{\opt}{\text{\sc opt}\xspace}
\newcommand{\e}{\varepsilon}
\renewcommand{\d}{\delta}
\renewcommand{\Pr}{\text{\bf Pr}\xspace}
\newcommand{\Ex}{\text{\bf Ex}\xspace}
\newcommand{\eat}[1]{}

We prove the following:

\begin{theorem}\label{thm:lower}
    For any $\gamma \in (0, 1)$, if a randomized algorithm \alg for the online Santa Claus problem with random order input satisfies 
    \[
        \alg \ge (1-\gamma) \cdot \opt,
    \]
    then $\opt \ge \frac{C \ln n}{\gamma}$ for some (absolute) constant $C > 0$.
\end{theorem}

We use the following construction. There are $n$ agents of which $n-1$ are {\em private} agents and the remaining one is a {\em public} agent. Every private agent has $k$ distinct private items for which their valuation is $1$ each, and the valuation of every other agent $0$. In addition, there are $k$ public items for each of which the valuation of every agent is $1$. The optimal solution is to assign the private items to the corresponding private agents, and the public items to the public agent. Thus, $\opt = k$.

Now, when the items are presented in uniform random order, consider the first $\e$ fraction of presented items -- call this the $\e$-prefix. Our main claim is that with constant probability, both of the following statements hold: (a) there are about $\e$ fraction of public items in this $\e$-prefix, and (b) there is at least one type of private item that is missing from this $\e$-prefix. For property (a), we need the following concentration inequality from Devanur and Hayes~\cite{devanur2009adwords}:
\begin{lemma}[Lemma 3 in \cite{devanur2009adwords}]\label{lem:dh}
     Let $Y = (Y_1, \ldots, Y_m)$ be a vector of real numbers, and let $0 < \e < 1$. Let $S$ be a random subset of $[m]$ of size $\e m$, and set $Y_S := \sum_{j\in S} Y_j$. Then, for every $0 < \d < 1$,
     \[
        \Pr\left[|Y_S - \Ex[Y_S]| \ge \frac{2}{3} \|Y\|_\infty \ln \left(\frac{2}{\d}\right) + \|Y\|_2 \sqrt{2\e \ln \left(\frac{2}{\d}\right)}\right] 
        \le \d.
    \]
\end{lemma}
Property (a) about the fraction of public items in the $\e$-prefix follows almost immediately from the above lemma:
\begin{lemma}\label{lem:public}
     The probability that there are fewer than $\frac{5\e}{12}$ fraction of public items in the $\e$-prefix is at most $2 e^{-\frac{\e k}{8}}$.
\end{lemma}
\begin{proof}
    We invoke \Cref{lem:dh} with the following setting of variables. Let $Y$ be a binary vector where $Y_i = 1$ for $i\in [k]$ and $Y_i = 0$ otherwise. ($Y_i$ is the indicator for whether an item is a public item.) $S$ represents the set of indices in the $\e$-prefix. Then, $Y_S$ counts the number of public items in the $\e$-prefix in a random ordering of the items. Clearly, $\Ex[Y_S] = \e k$, $\|Y\|_\infty = 1$, and $\|Y\|_2 = \sqrt{k}$. Finally, set $\d = 2 e^{-\frac{\e k}{8}}$, i.e., $\ln \left(\frac{2}{\d}\right) = \frac{\e k}{8}$. Now, by \Cref{lem:dh}, we have
    \[
        \Pr\left[|Y_S - \e k| \ge \frac{2}{3} \cdot \frac{\e k}{8} + \sqrt{k}\cdot \sqrt{2\e \cdot \frac{\e k}{8}}\right] 
        = \Pr\left[|Y_S - \e k| \ge \frac{7}{12} \cdot \e k\right] 
        \le 2 e^{-\frac{\e k}{8}}.
    \]
    The lemma follows.
\end{proof}

Now, we show property (b) about the non-existence of at least one type of private item in the $\e$-prefix.
\begin{lemma}\label{lem:private}
    The probability that all the $n-1$ types of private items appear in the $\e$-prefix is at most $e^{-4^{-\frac{\e}{1-\e} k}(n-1)}$.
\end{lemma}
\begin{proof}
    Fix a type of private item, say those of type-$j$, i.e., only agent $j$ (for some $j\in [n-1]$) has unit value for this type of item while all other agents have $0$ value. First, we bound the probability that no item of type-$j$ appears in the $\e$-prefix. To do this, note that this probability can be written, using the chain rule for conditional probabilities, as the product (over $i$ from $1$ to $\e nk$) of the probabilities of the $i$th item in the $\e$-prefix not being a type-$j$ item under the condition that the first $i-1$ items were not type-$j$ items either. Clearly, this probability, for any $i\le \e nk$, is at least $1-\frac{1}{(1-\e)n}$ since there are $k$ items of type-$j$ among at most $(1-\e)nk$ items overall after the conditioning. Thus, the probability that no item of type-$j$ appears in the $\e$-prefix is at least
    \[
        \left(1-\frac{1}{(1-\e)n}\right)^{\e nk} \ge 4^{-\frac{\e}{1-\e}\cdot k} \text{ by choosing } n \ge \frac{2}{1-\e}.
    \]
    Denote $p = 4^{-\frac{\e}{1-\e}\cdot k}$. Consider the events that at least one item of type-$j$ appears in the $\e$-prefix. These events are negatively correlated. Therefore, the probability that at least one item of type-$j$ appears in the $\e$-prefix for every $j\in [n-1]$ is at most
    \[
        (1-p)^{n-1} 
        \le \left(1-4^{-\frac{\e}{1-\e}\cdot k}\right)^{n-1}
        \le e^{-4^{-\frac{\e}{1-\e} k}(n-1)}.
    \]
\end{proof}

Now, choose 
\begin{equation}\label{eq:k}
    k = \frac{1-\e}{2\e} \cdot \lg (n-1).
\end{equation}
Then, 
\[
    4^{-\frac{\e}{1-\e} k} (n-1)
    = 2^{-\frac{2\e}{1-\e} \cdot \frac{1-\e}{2\e}\cdot \lg (n-1)} (n-1)
    = 2^{-\lg (n-1)} (n-1)
    = 1,
\]
and 
\[
    \frac{\e k}{8} = \frac{1-\e}{16}\cdot \lg(n-1).
\]
Plugging these expressions into \Cref{lem:private} and \Cref{lem:public}, we get that the probability of every private item type appearing in the $\e$-prefix is at most $\frac1e$ and that of fewer than $\frac{5\e}{12}$ fraction of public items appearing in the $\e$-prefix is at most $2 e^{-\frac{1-\e}{16}\cdot \lg(n-1)}$. The latter probability can be further simplified to
\[
    2 e^{-\frac{1-\e}{16}\cdot \lg(n-1)}
    = 2 e^{-\frac{1-\e}{16}\cdot \frac{\ln(n-1)}{\ln 2}}
    = \left(\frac{2}{n-1}\right)^{\frac{1-\e}{16\ln 2}}
    < \frac1e \text{ for large enough } n.
\]
Using the union bound over these two events, we conclude that with probability at least $1-\frac2e$, there is at least one missing private item type in the $\e$-prefix, and also at least $\frac{5\e}{12}$ fraction of private items appear in the $\e$-prefix. In this case, in the $\e$-prefix, the algorithm cannot distinguish between the private agent whose item type is missing and the public agent. Thus, in expectation (over the randomness of the algorithm), at least half the public items in the $\e$-prefix are assigned to the private agent whose item type is missing. As a consequence, at least $\frac{5\e}{24}$ fraction of the public items are not allocated to the public agent in the entire algorithm, which means that the total valuation of the public agent is at most $\left(1 - \frac{5\e}{24}\right) k$.

Thus, in order to get 
\[
    \alg \ge (1-\gamma)\cdot \opt,
\]
we need $\gamma \ge \frac{5\e}{24}$, i.e., $\frac1\e \ge \frac{5}{24\gamma}$. This implies by \Cref{eq:k} that
\[
    \opt
    = k 
    = \frac{1-\e}{2\e}\cdot \lg (n-1)
    = \frac{\frac1\e-1}{2}\cdot \lg (n-1)
    \ge \frac{\frac{5}{24\gamma}-1}{2}\cdot \lg (n-1)
    \ge C\cdot \frac{\ln n}{\gamma} \text{ for some constant } C.
\]
This completes the proof of \Cref{thm:lower}.\qed

==> TrashFiles/introduction.tex <==
Fair allocation of resources is one of the central themes of algorithmic game theory. In fact, the theory of fair division has its roots in mathematics going back to as early as 1948~\cite{steihaus1948problem}. In the general setting, this problem comprises a set of items that must be divided among a set of agents in an egalitarian manner, where each agent has a (possibly non-uniform) valuation for each item. A natural objective to capture the goal of egalitarian or fair division is to maximize the minimum total value of items received by any agent. This gives rise to the famous ``Santa Claus problem'' that we describe below.

In the Santa Claus problem, originally described by Bansal and Sviridenko in 2006 \cite{Bansal_2006} (although it was studied under different names or assumptions prior to this), the Santa Claus is said to have a set of $m$ presents to be distributed equitably among $n$ children. Each child $i\in [n]$ has some arbitrary non-negative value $v_{ij}$ for present $j\in [m]$. Furthermore, Santa's goal is to distribute the presents in a way that makes the least satisfied child maximally satisfied. More formally, this means that the assignment seeks to maximize the minimum total value of the presents received by any child, where the total value of presents received by a child is the sum of her values for the presents that she received. The Santa Claus problem can be formalized as the following integer program:
%
\begin{gather*}
\max \lambda \\
\begin{aligned}
\textup{s.t.}\quad &\forall i \in [n] &\quad \sum_{j=1}^m v_{ij} \cdot x_{ij}  \geq  \lambda \\
            &\forall j \in [m] &\quad \sum_{i=1}^n x_{ij} \le 1\\
            &\forall i\in [n], j\in [m] &\quad x_{ij} \in \{0, 1\}
\end{aligned}
\end{gather*}
where $x_{ij}$ is the indicator variable for assigning the $j$-th present to the $i$-th child.

The general case of this problem was initially explored (under a different name) in the field of algorithmic game theory for the fair allocation of goods \cite{lipton2004approximately}. By studying the assignment LP of \cite{lenstra1990approximation} for the dual ``makespan'' problem, Bezakova and Dani \cite{bezakova2005allocating} derived an additive approximation of $\max_{ij} v_{ij}$, i.e., the objective in the algorithm's solution is at least $\opt - \max_{ij} v_{ij}$ where \opt{} is the objective value of the optimal solution. They also extended the hardness result on the dual makespan minimization problem~\cite{lenstra1990approximation} to demonstrate that the Santa Claus problem is NP-hard and cannot be approximated to a factor better than 2. Later, Bansal and Sviridenko~\cite{Bansal_2006} demonstrated that the integrality gap of the configuration LP for this problem is $\Omega(\sqrt{n})$, while Asadpour and Saberi~\cite{Asadpour_2010} complimented this result with a $O(\sqrt{m} \log^3 m)$ upper bound for the same LP relaxation. To date, the best algorithmic result for the Santa Claus is an $\tilde{O}(n^\ve)$-approximate algorithm, where $\ve = \Omega(\log \log n / \log n)$, in quasi-polynomial time obtained by Chakrabarty, Chuzhoy, and Khanna~\cite{ChakrabartyCK09}.

For the special case of \emph{restricted assignment}, i.e. $v_{ij} \in \{0,v_j\}$, Bansal and Sviridenko \cite{Bansal_2006} provided an $\Omega \left(\frac{\log \log \log m}{\log \log m}\right)$-approximate algorithm that relies on rounding a configuration LP. Later, Feige showed that this LP relaxation actually has only an $O(1)$ integrality gap, although this result was non-constructive~\cite{feige2008allocations}. Asadpour, Feige, and Saberi~\cite{Asadpour_2012} made this constructive in that they obtained an approximation factor of $1/4$ via a rounding algorithm based on local search, but the algorithm is not known to converge in polynomial time. Further work has since improved this constant factor \cite{jansen2018note,cheng2018restricted,davies2019tale,annamalai2016combinatorial}, improved upon the running time \cite{cheng2019restricted}, and further extended the setting beyond additive valuations \cite{bamas2020submodular}.


% \alert{We need the full history of the Santa Claus problem here, including work before Bansal and Sviridenko mentioning that it arose originally in the algorithmic game theory community -- see their paper. The stuff about related problems like the min-max objective should be postponed to related work.}

\eat{

The objective here is contrasted in the allocation problem literature with that of maximizing the \emph{total} utility of all competing agents in a system, a naturally simpler problem. To be precise, we can formalize our problem with the following offline linear program:
%
\begin{gather*}
\max \lambda \\
\begin{aligned}
\textup{s.t.}\quad &\forall i \in \mathcal{N} \quad \sum_{j \in \mathcal{S}_i} v_{ij} \cdot x_{ij}  \geq  \lambda \\
            &\forall j \in \mathcal{M} \quad \sum_i x_{ij} \leq 1
\end{aligned}
\end{gather*}
where $x_{ij}$ denotes the fraction of item $j$ assigned to person $i$ and $\mathcal{S}_i$ is the subset of items allocated to $i$. In this work, we further reduce the problem to that of unit values: $v_{ij} \in \{0,1\}$ for all $j \in \mathcal{M}$.

Allocation problems are fundamental throughout our daily lives and have recently become increasingly critical with the advent of the internet, with interest being drawn from mathematicians as early as 1948 \cite{steihaus1948problem}. The goal of evenly distributing a good or set of goods across individuals seemingly arises in many fields and as such is of great interest for mathematicians and computer scientists alike. In spite of their longstanding history, the remarkable difficulty of solving such problems within many different contexts has allowed for many questions to be still unanswered or even unexplored in the literature to date.
%
Resource allocation problems specifically, wherein limited resources need to be allocated to agents subject to given system constraints, are at the core of the field of algorithmic game theory and as such have been studied for decades in the fields of computer science, economics and mathematics with the bulk of results coming in the form of approximations to an optimal solution. These problems can be further subdivided into the divisible and indivisible problem instances, further extending the problems into both the continuous and discrete settings (each requiring unique algorithmic strategies towards solutions). 

Most recently, these allocation problems have been further extended to the online setting, where items need to be irrevocably allocated at the moment that their information is obtained. This setting is highly practical as a means to accommodate rising importance of algorithms that perform well in real-time implementation on the internet \cite{Buchbinder_2007,Blum_2006,Hajiaghayi_2007,Zhou_2008}. 
%
In the present work, we restrict our attention to the egalitarian objective allocation in the ``Santa Claus'' (sometimes referred to as the \textsc{MaxMin}) problem and present its novel extension to the online input setting. Most importantly, we present upper and lower bounds for the problem under differing input regimes that are nearly tight.

The Santa Claus problem is a known NP-hard problem that was originally described by Bansal in 2006 \cite{Bansal_2006} and has given rise to a rich literature of progressive improvements on the hardness and algorithmic guarantees for the offline allocations \cite{Asadpour_2010,Davies_2020,Dwork_2012,Feldman_2010,Svensson_2012}. In this allocation problem, the Santa Claus is said to have a set $\mathcal{M}$ of $m$ presents to be partitioned and distributed equitably across $n$ children where every child has some arbitrary value for each present $v$. Furthermore, Santa's goal is to distribute the presents such that the child who receives the bundle of \emph{minimal} value has the \emph{maximal} possible value for the given input. This is the so-called \textsc{MaxMin} objective, which has been also been studied in the ``machine covering'' problem \cite{Azar_1998,Epstein_2011,Epstein_2018,Svensson_2012}, or in its dual form (\textsc{MinMax})
as the ``makespan'' problem \cite{Chakrabarty_2014,Gupta_2014,Molinaro_2017}. The objective here is contrasted in the allocation problem literature with that of maximizing the \emph{total} utility of all competing agents in a system, a naturally simpler problem. To be precise, we can formalize our problem with the following offline linear program:
%
\begin{gather*}
\max \lambda \\
\begin{aligned}
\textup{s.t.}\quad &\forall i \in \mathcal{N} \quad \sum_{j \in \mathcal{S}_i} v_{ij} \cdot x_{ij}  \geq  \lambda \\
            &\forall j \in \mathcal{M} \quad \sum_i x_{ij} \leq 1
\end{aligned}
\end{gather*}
where $x_{ij}$ denotes the fraction of item $j$ assigned to person $i$ and $\mathcal{S}_i$ is the subset of items allocated to $i$. In this work, we further reduce the problem to that of unit values: $v_{ij} \in \{0,1\}$ for all $j \in \mathcal{M}$.

For the original offline problem, Chakrabarty et al \cite{ChakrabartyCK09} provided an $\tilde{O}(n^{\ve})$ approximate solution for any $\ve = \Omega(\log \log n / \log n) $ in poly-logarithmic time, invoking a linear program that demonstrates a $\Omega(\sqrt m)$ integrality gap. Additionally, Asadpour and Saberi \cite{Asadpour_2010} provided the first polynomial time approximate solution that was further improved upon in \cite{Haeupler_2011}. More recently, Asadpour et al \cite{Asadpour_2012} provided the first constant factor approximation via a configuration LP for the problem. While these results have produced great strides on solutions to the problem, they more so demonstrate the tremendous complexity of this problem in the offline setting, a fact which spills over into the potential competitive ratio guarantees of the online extension in the form of an additive loss factor.

}%end eat

% \debmalya{I am not sure I follow the next paragraph. Can you please clarify what you mean in the advertising example for instance?}
In many situations, however, the entire set of items that can be allocated is not known in advance. For example, in online advertising, ad-space providers will receive monetary bids from competing agents for the display of their advertisements in real-time for an available space on a webpage \cite{Buchbinder_2007,Blum_2006,Hajiaghayi_2007,Zhou_2008}. As such, the provider must make irrevocable decisions as to which advertiser's bid to accept for the display of their ad to ensure that revenue is maximized only using knowledge of prior allocations and the current bids for the available space \cite{balseiro2019learning,conitzer2021multiplicative}. Beyond advertising, online allocation procedures have been critical in the study of donation distribution, wireless charging networks and especially organ donor matching (see \cite{aleksandrov2020online} for exhaustive survey on these applications). 

Motivated by these applications, we consider the {\em online} Santa Claus problem in this paper. In this problem, the items arrive in an online sequence and must be allocated to one of the agents immediately on arrival. As in the offline problem, our goal is to maximize the minimum total value among all agents. %While the problem may seem like a trivial extension, in practice it increases the complexity tremendously. 
To illustrate the problem, consider the simple example in Figure \ref{fig:hard_ex}. At the time of the first arriving item, all agents can be matched to this item and therefore with probability $\frac{1}{3}$ the rightmost agent will receive it. However, as we continue forward with the input stream, we see in retrospect that the only nonzero max-min solution can be achieved if that first item was indeed allocated to the rightmost agent (as it is the only possible item they can receive). %In the offline instance, it is very easy to see this solution, but the incremental reveal of information requires both sophisticated algorithms and assumptions on the input instance that diminish the possibility of such complexity.

\begin{figure}[t]
	\includegraphics[width=0.6\textwidth]{figures/hardness.png}
	\caption{Example online problem instance. Fixed agents are presented in the top row and the arriving items are arranged from left to right in correspondence with their arrival order. Edges indicate a nonzero item valuation to a given agent, i.e. a possible assignment.}
	\label{fig:hard_ex}
\end{figure}

Following standard terminology for online algorithms (see, e.g., \cite{borodin2005online}), we define the {\em competitive ratio} of an online algorithm as the minimum ratio between the value of the (maximization) objective in the algorithm's solution to that in the optimal (offline) solution in hindsight. We furthermore discuss the \emph{additive regret} as the additive loss factor of our algorithm. More formally, we say our algorithm, \alg, has competitive ratio $c$ and additive regret $b$ if these are the largest and smallest values respectively that satisfy
$$\alg \geq c \cdot \opt{} - b.$$

Prior work on the max-min objective in the online setting allowed various relaxations of the problem, such as allowing for some reordering in the allocation process \cite{Epstein_2011}, restricting the number of agents \cite{he2005optimal,tan2006semi,wu2014optimal}, or allowing migration of items after assignment \cite{chen2011line}. This is because of two reasons. First, even in the offline setting, there remains a huge gap between the best upper and lower bounds on the approximation ratio of the Santa Claus problem, and bridging this gap is a major open problem. Second, as we will soon see, there is a simple construction for the online problem that shows the competitive ratio cannot be better than $n$. To bypass these bottlenecks, our first assumption in this paper is that the items arrive in {\em random order}. This is a standard assumption that has been used for many online problems such as budgeted allocation \cite{devanur2009adwords,feldman2009online,goel2008online}, online matching \cite{feldman2009online2,karande2011online}, secretary problems \cite{babaioff2007knapsack,kleinberg2005multiple}, and so on. But, even with this assumption, we show that obtaining a competitive solution is impossible in general {\em for small problem instances}. This motivates our second assumption: that the objective value of the optimal solution is sufficiently large. In fact, we obtain the precise threshold on the optimal objective in the random order setting. With these two assumptions, we give an algorithm that obtains a competitive ratio of $(1-\e)$ for any $\e > 0$. We note that using standard techniques, the assumption about the optimal objective being sufficiently large can be replaced by a corresponding additive regret in the competitive ratio.
%These works in general only consider worst case guarantees, with the studies on the more relaxed input settings for the general MaxMin problem being limited.
  
 % More recently, Kawase and Sumita \cite{Kawase_2021} studied the \textsc{MaxMin} problem without these budgeting constraints and also demonstrated a $(1-\ve)$ competitive ratio in the i.i.d. setting. While the authors achieve this result with a unique multiplicative weights update approach in line with \cite{Devanur_2011}, they ultimately do not provide an extension beyond the results presented in \cite{Gollapudi_2014}. Specifically, the authors reiterate that an important extension would be to assume a random-order input model while noting that such results can likely only be achieved by proving a lower bound on the offline hardness of the input instance. Our paper proceeds by presenting exactly these results and achieves this by a simple approximately greedy approach. \todo{maybe not necessary to discuss this preprint, but their lack of novel results do further bolster ours?}


We now formally define the two online input stream models that we talk about in this paper: \emph{adversarial} and \emph{random order} input.

\begin{definition}[Adversarial Input]
An adversary selects the value vector $v \in [0,1]^n$ of each arriving item for all the agents, as well as the order in which these vectors arrive.
\end{definition}
\begin{definition}[Random-Order Input]
An adversary selects the value vector $v \in [0,1]^n$ of each arriving item for all the agents, but these vectors are randomly permuted to determine their arrival order.
\end{definition}

Note that in the literature, the independent and identically distributed (i.i.d.) input model is also often studied for related problems \cite{goel2008online,karp1990optimal,mahdian2011online,karande2011online,Agrawal_2014,kesselheim2014primal,seiden2002online,molinaro2014geometry}. In this model, the adversary picks a distribution over inputs that is unknown to the algorithm and arriving items are sampled i.i.d. from this distribution. The random order model is {\em stronger} than the i.i.d. model in the sense that any algorithmic result for the random order model automatically extends to the i.i.d. setting as well. This includes the algorithmic results that we obtain in this paper for the random order arrival model. %As a result, any algorithm that works for the random order input will also work on an i.i.d. input. We thus assume these results, but do not formally consider them in the main text. 

\eat{
Building on these foundational works, we here provide an extension to the \emph{online} Santa Claus problem, wherein the items to be allocated arrive as a continuous stream. Crucially, we provide nearly optimal algorithms for the random-order and weaker i.i.d. input settings as well as a tight matching lower-bounding counter example on the offline solution in order to achieve the optimal online result. We additionally examine the worst-case analysis for the problem instance, which is completely robust to input uncertainty. This setting allows for only pessimistic performance bounds on an online algorithm that are far from optimal, further justifying the relaxation to the random order model. In spite of the increased complexity for an adversarial input, we further prove tight upper and lower bounds with respect to a stronger assumption on the input instances.
}%end eat

\subsection{Our Results} \label{sec.our_work}
\eat{
While the Santa Claus problem has been studied extensively in the offline setting, the analysis of a competitive ratio in the online setting is almost entirely unexplored. Traditionally, algorithmic guarantees under the adversarial input model, where an adversary selects both the item vector values $v \in \{0,1\}^n$ and the order in which they arrive, are far from optimal. In Theorem \ref{thm:ad-upper}, we demonstrate that the online Santa Claus problem is no exception and verify the result with a simple proof.
}
First, we give a simple construction to show that if the arrival order of the items is adversarial, then the best competitive ratio that can be achieved is only $1/n$. (In fact, we also match with competitive ratio using a simple algorithm in the appendix.)
\begin{theorem}[Adversarial Input] \label{thm:ad-upper}
    In the adversarial setting, no algorithm can obtain a competitive ratio better than $\frac1n$.
\end{theorem}
\begin{proof}
    We consider the following instance: of the $n$ agents, $n-1$ are \emph{private} agents each having $k$ private items that have valuation $1$ for the corresponding private agent and $0$ for every other agent. The $n$-th agent is a \emph{public} agent and there are $k$ public items that have a valuation of $1$ for all the $n$ agents. A graphical depiction of these two item types is presented in Figure \ref{fig:item_types}.
    
    The optimal solution assigns the private items to the corresponding private agents and the public items to the public agent. Thus, $\opt = k$. In the online instance, the adversary chooses to present all the public items before the private items. Since all the agents look identical before the arrival of the first private item, the public agent gets no more than $k/n$ items in expectation for any algorithm (this adversarial input is comparable to our toy example discussed in Figure \ref{fig:hard_ex}). Since none of the remaining private items can be allocated to the one public agent, their bundle value can no longer increase beyond $k/n$. The theorem follows.
\end{proof}

\begin{figure}[t]
	\includegraphics[width=\textwidth]{figures/item_types3.png}
	\caption{Public and private item type construction. The top nodes indicate the (offline) agents and the bottom is the arriving item. Edges indicate a nonzero item valuation to a given agent, i.e. a possible assignment.}
	\label{fig:item_types}
\end{figure}

\eat{
As a consequence of this negative result, we instead turn our attention to the \emph{random order model}, wherein an adversary again selects the input stream, but not the order in which it is presented. Our primary result demonstrates an optimal $(1-\ve)$-competitive ratio for the random order input models, subject to conditions on the input instance that we prove to be tight. We thus show that while the adversarial input allows for only weak guarantees in the online setting, the relaxation to a random order input stream allows for an optimal solution assuming the input instance is sufficiently large. Our main results are stated in Theorems \ref{thm:main_ROM} and \ref{thm:main_lower}, and these results are contrasted against the literature on the \emph{offline} problem instance in Table \ref{tab:one}.
}

As a consequence of this negative result, we instead turn our attention to the \emph{random order model}, wherein an adversary again selects the input stream, but not the order in which it is presented. The main contribution of our paper is to propose an algorithm that produces a fractional solution that achieves a nearly optimal competitive ratio in this relaxed input model, a first result of this kind. This result is achieved by a smoothing of the minimum function, which we will allocate with respect to, as well as a ``restart'' on the allocation values halfway through the input stream to alleviate the correlations that arise between items. Crucially, we also demonstrate a necessary dependence on the input instance size to allow for a $(1-\ve)$-competitive ratio. This result is stated precisely as follows:

\begin{theorem}[Random Order: Algorithm] \label{thm:main_ROM}
    For any $\ve > 0$, there is an online algorithm for the Santa Claus problem that has a competitive ratio of $(1 - \ve)$ in the random order input model for all input instances such that the value of the optimal offline solution satisfies $\opt{} \geq \Omega \left( \frac{\log n}{\ve^2} \right)$.
\end{theorem}

Our complimentary result comes in the form of an impossibility result for algorithms in the random order input model. We show that the minimum bound on $\opt$ is required and that the dependence on $n$ is precisely the correct one. The dependence on $\ve$ is $\frac1\ve$ in the impossibility result and $\frac{1}{\ve^2}$ in the algorithm; bridging this gap is an interesting open question.

\begin{theorem}[Random Order: Impossibility Result] \label{thm:main_lower}
    For any $\ve \in (0, 1)$, there is no online algorithm for the Santa Claus problem in the random order input model that has a competitive ratio of $(1-\ve)$ when $\opt < C\cdot \frac{\ln n}{\ve}$ for some (absolute) constant $C > 0$.
\end{theorem}

% \alert{next para is very vague, needs rewriting, what is the problem you are comparing to?}
%We further note that the condition on the input instance size in Theorems \ref{thm:main_ROM} and \ref{thm:main_lower} is theoretical, and our algorithm may still achieve a strong competitive ratio if the conditions are not exactly satisfied in practice. Thus, our main results are both theoretically and practically important in the online space.

Our results for the online problem are collected and contrasted against the well-studied offline problem in Table \ref{tab:one}.

\eat{
\alert{again, very sketchy, try to rewrite}
Our results on the optimal solution proceeds in the following manner: we define a re-scaled variant of the \textsc{LogSumExp} function that is a smoothed version of the minimum function and prove various properties that are essential to maintaining a low additive error loss throughout the allocation procedure. We define our algorithm to make greedy assignments with respect to this functions accumulated value, implementing a ``restart'' on the procedure half-way through the input stream (thus, the algorithm assumed knowledge of $m$) to alleviate the the correlation that arises in the random order input sampling. We subsequently bound the total error accumulated both before and after the restart using a similar methodology to that of \cite{AgraDev_2014}, and lastly combine these two bounds to get the final competitive guarantee as compared to the optimal offline allocation decisions.
}

\begin{table}[t]
	\caption{Santa Claus Problem Results}
	\label{tab:one}
	\begin{minipage}{\columnwidth}
		\begin{center}
		    \begin{tabular}{ccc}
		    % Centered offline break
		    & \textbf{Offline Results} & \\
			\toprule
			Paper & Algorithm & Approximation Ratio \\
				\toprule
				Bansal and Sviridenko \cite{Bansal_2006} & Configuration LP  & $\Omega \left( \frac{\log \log m}{\log \log \log m} \right)$\\
				Asadpour and Saberi \cite{Asadpour_2010} & Tree Matching  & $\Omega\left( \frac{1}{\sqrt{n} \log^3 n} \right)$\\
				Chakrabarty et al. \cite{Chakrabarty_2009} & Configuration LP  & $\tilde{O} \left( n^\ve \right)$, $\ve = \Omega \left(\frac{\log \log n}{\log n}\right)$\\
				Asadpour et al. \cite{Asadpour_2012} & HyperGraph Matching  & $\frac{1}{4}$\\[1.5mm]
			\toprule
			% Centered Online Break
			& \textbf{Online Results} & \\
			& \small\small{(This Paper)} & \\
			\bottomrule
			Input Model & Algorithm & Competitive Ratio \\
				\toprule
				Adversarial Input & \textsc{Random}  & $\left(\frac{1-\ve}{n}\right)\opt{} - O\left(\frac{n \log n}{\ve^2}\right)$\footnote[1]{Proof deferred to the appendix.}\\
				Random Order & \textsc{SmoothGreedyWithRestart} & $(1-\ve) \opt - O \left(\frac{\log n}{\ve}\right)$ \\
				\textsc{IID} & \textsc{SmoothGreedyWithRestart} & $(1-\ve) \opt - O\left(\frac{\log n}{\ve}\right)$\\
				\bottomrule
			\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%

% With the advent of internet advertising and online sales, these allocation problems have become pivotal in the revenue maximization and fair distribution of virtual space for major companies like Amazon, Google and Facebook to name a small fraction. As such, we contextualize the assignment problem within online  advertising systems. In this domain, impressions arrive over time (in an online manner) and interested advertisers (bidders) submit bids based on how they value each impression. While this problem has been studied extensively for the purpose of revenue maximization \cite{Buchbinder_2007,Blum_2006,Hajiaghayi_2007,Zhou_2008}, we here consider efficient algorithms that retain a certain degree of \emph{fairness} to the competitive advertisers.

% -------------------------------------
\subsection{Preliminaries and Outline} % Notational definitions only, bring random order algo stuff up here
We here define some notation specific to the input model. Let $\bA^1, ..., \bA^m$ denote the input sequence of items arriving in random order where each $\bA^j$ is an $n \times n$ matrix defining the value vectors of the impression to each agent. More concretely, let $\bA_{i}^j$ denote the $i$-th column of such a matrix which represents the value of impression $j$ to agent $i$. Furthermore, this vector can only have a nonzero value in the $i$-th position: $\bA_{i}^j = (0,...,0,v_{ij},0,...,0)^T$. We again note that in the random-order input model, an adversary selects each of the $\bA^j$ but is not permitted to select the \emph{order} that they arrive in. This allows for substantially improved guarantees over the adversarial input model. We additionally let $\bx^1, ... , \bx^m \in [0,1]^n$ denote the allocation decisions output by the algorithm which are compared against the allocations made by the optimal offline solution, $\xopt^1, ..., \xopt^m \in [0,1]^n$ and further let $\opt{}$ denote the optimal offline solution for the given instance. Lastly, we let $\bv^t = \sum_{\tau=1}^t \bA^\tau \bx^\tau = (v_1^t, ..., v_n^t)$ be the vector of agent's allocation values up to time $t$. Our problem thus amounts to maximizing the component-wise minimum of $\bv^m$.

\eat{
We here concretely define the online setting input, where items to be allocated arrive one at a time and need to be permanently assigned to an agent upon arrival. More specifically, at time $t$ the algorithm is shown item value vector $v_t \in \{0,1\}^n$ and must decide on the receiving agent, based only upon the previous $t-1$ item decisions, prior to seeing the $t-1$-th item. We will examine this problem under the adversarial, random-order and i.i.d. frameworks defined as follows: \todo{not sure if these definitions are necessary, and more so if they should be moved to before our theorem statements on these inputs}
\begin{definition}[Adversarial Input]
An adversary selects the value vector $v \in \{0,1\}^n$ of each arriving item to all agents, as well as the order in which these vectors arrive.
\end{definition}
\begin{definition}[Random-Order Input]
An adversary selects the value vector $v \in \{0,1\}^n$ of each arriving item to all agents, but these vectors are subsequently randomly permuted to determine their arrival order.
\end{definition}
\begin{definition}[\textsc{IID} Input]
Item vector values are randomly sampled i.i.d. from an unknown distribution, $v \sim \mathcal{D}^n$, at each arrival time step where the adversary has selected the distribution.
\end{definition}
As such, the adversarial input is the hardest to achieve positive result for, whereas the random-order and i.i.d. models are naturally more predictable and thus allow for improved guarantees. In each setting, we prove results on the worse possible inputs so as to demonstrate the robustness of our algorithms, however in practice it may not be the case that these worst-case inputs arise. As such, even for the less impressive competitive ratio results, our algorithms may still perform better than the theoretical guarantee.

In discussing the hardness of the above input contexts, we assess the quality of our algorithms by their \emph{competitive ratio}, or the ratio of our online algorithm's solution to that of the optimal \emph{offline} solution (denoted \opt{}). More formally, let $\mathcal{I}$ denote an arbitrary input instance and \alg denote the solution value output by the designed online algorithm, then the competitive ratio is at least $c$ when there exists some constant $b \geq 0$: $$\alg(\mathcal{I}) \geq c \cdot \opt{}(\mathcal{I}) - b$$
Furthermore, under the random-order and i.i.d. input models we must consider the \emph{expected} value of the algorithm over the possible online stream input instances. Thus, the competitive ratio is often defined in the random-order model as
$$\inf_{\mathcal{I}} \frac{\Ex[\alg(\mathcal{I})]}{\opt(\mathcal{I})}$$
and for the i.i.d. input as
$$\inf_{\mathcal{\sigma} \sim \mathcal{I}} \frac{\Ex_{\mathcal{\sigma} \sim \mathcal{I}}[\alg(\sigma)]}{\Ex_{\mathcal{\sigma} \sim \mathcal{I}}[\opt(\sigma)]}$$
where $\mathcal{I}$ is now an unknown distribution. It is important to note that the optimal offline solution in the random-order model is \emph{not} changing in the instances, as the impressions are fixed and their arrival order does not impact the offline setting.
}

The remainder of the paper is organized as follows: in Section \ref{sec.related} we discuss the literature on related problems and how the present work compares, in Section \ref{sec.algo} we present a $(1 - \ve)$-competitive algorithm for the random order model and in Section \ref{sec.bounds} we compliment these results with novel impossibility results on the Santa Claus problem. We lastly provide concluding remarks in Section \ref{sec.con}.

\section{Related Work}\label{sec.related}
The study of allocation and assignment problems is expansive, garnering wide interest in the fields of computer science, operations research and management sciences to name a few. In the online algorithms research, many of the preliminary results emphasized only the worst case bounds and adversarial input models \cite{Azar_1998,Ebenlendr_2005}, however the random order (or permutation) model has recently experienced a bump in popularity due to its necessarily improved guarantees on the worst case. Various online problems have been examined under this improved model such as the secretary problem \cite{babaioff2007knapsack,kleinberg2005multiple}, AdWords \cite{devanur2009adwords,feldman2009online,goel2008online}, online matching \cite{feldman2009online2,karande2011online}, online packing \cite{Gupta_2014,feldman2010online,kesselheim2014primal}, and makespan or load-balancing (the dual equivalent to our problem) \cite{Molinaro_2017,Liu_2021}. In this section, we focus on a few of these related problems and how they relate to the Santa Claus.
%
\vspace{2.5mm}\\
\noindent \textbf{MaxMin.} Though the studies on the online maxmin under non-worst case inputs is very limited, there exists some prior results on the problem. One such study is that of \cite{Gollapudi_2014} which considered this problem with added packing constraints, among other fairness objective functions for the purpose of revenue maximization. The work presents a nearly optimal $(1-\ve)$-competitive algorithm for the i.i.d. input setting but, despite this positive result, the authors do not extend their results to the more complex and practical \emph{random order model}, a novel result presented in our paper. Furthermore, while the authors make the assumption that the optimal offline solution is lower bounded as $\Omega \left(\frac{\log n}{\ve} \right)$ they do not provide a proof on the necessity of such an assumption, a point that we make clear in the present work.
%
\vspace{2.5mm}\\
\noindent \textbf{Makespan.} Closely related to our problem is that of the online ``makespan'' (also known as load balancing or scheduling) problem which considers the dual objective of minimizing the maximal bundle value from online assignment, having been studied as early as the 1960s \cite{graham1966bounds,liu1973scheduling}. A recent relevant work is that of Molinaro \cite{Molinaro_2017} which studies this problem, building upon prior results for the experts approach \cite{Gupta_2014}. This work examines algorithms that work well in both the adversarial and random-order model, balancing the hardness of the two distinct input streams to achieve a ``best of both worlds'' result. In achieving this, the authors relax the maximum function to a general $L^p$ norm and analyze the problem as it depends on the parameter $p$. We here extend their results by emulating the proof technique for the \emph{concave} objective function of a smoothed minimum. Further work by \cite{Liu_2021} demonstrated that the greedy allocation procedure is necessarily optimal for the makespan problem without giving the exact competitive ratio of this algorithm. As we will demonstrate in our competitive ratio analysis, our results are effectively the dual compliment to the prior work. While in general minimization and maximization problem solutions do not align, we demonstrate that in this problem instance the two align well. 
%
\vspace{2.5mm}\\
\noindent \textbf{Packing.} Online packing LPs, where the arriving items are to be placed in bins that have some fixed limited capacity such that the items are fairly distributed without exceeding these capacities also closely matches the nature of our problem \cite{buchbinder2009online,buchbinder2005online,feldman2010online}. This problem has been extensively studied under all input models, with near optimal results being obtained for the random order and i.i.d. setting subject to constraints on the input size \cite{Agrawal_2014,kesselheim2014primal,seiden2002online,molinaro2014geometry}. Most relevant to our paper, \cite{Agrawal_2014} proves that, in the random order model, an algorithm can achieve a competitive ratio of $1-\ve$ if and only if the input packing constraints exceed $\Omega \left( \frac{\log n}{\ve^2} \right)$. This result is derived by a careful worse-case example construction, a method that we closely follow in the construction of our impossibility results for the current problem, though we only demonstrate the looser $\Omega \left( \frac{\log n}{\ve} \right)$ bound.
%
\vspace{2.5mm}\\
\noindent \textbf{Matching.} Online bipartite matching was originally presented by Karp et al. \cite{karp1990optimal} and involves a bipartite graph $G(U,V,E)$ where one side is known and the other side arrives in an online fashion. As the vertices arrive, its neighbors are revealed and the vertex must be matched to one of the available neighbors (if they exist). The objective is to maximize such a matching, and as a result the problem can effectively be seen as a sub-problem on the Santa Claus problem with unit value items and a capacity on each agent. The problem has been thoroughly studied in both the adversarial \cite{karp1990optimal,goel2008online,birnbaum2008line} and random order \cite{goel2008online,karp1990optimal,mahdian2011online,karande2011online} inputs, and has further been extended to the case of \emph{weighted} vertex matching where graph edges have a weight, $w$ \cite{aggarwal2011online,feldman2009online3,jaillet2014online}. The methodologies here provide key insight on our problem.

\eat{
The study of fair allocation problems is expansive, garnering wide interest in the fields of computer science, operations research and management sciences to name a few. In the online algorithms research, many of the preliminary results emphasized only the worst case bounds and adversarial input models, however the random order (or permutation) model has recently experienced a bump in popularity due to its necessarily improved guarantees on the worst case. Various online problems have been examined under this improved model such as the secretary problem \cite{babaioff2007knapsack,kleinberg2005multiple}, AdWords \cite{devanur2009adwords,feldman2009online,goel2008online}, online matching \cite{feldman2009online2,karande2011online}, online packing \cite{Gupta_2014,feldman2010online,kesselheim2014primal}, and makespan or load-balancing (the dual equivalent to our problem) \cite{Molinaro_2017,Liu_2021}. In this section, we focus on a few papers that focus on the competitive ratio and impossibility results with a nonlinear objective function as in our work.
%
% The problem of budgeted distribution of goods in an online distribution has a vast body of literature, mostly devoted to the objective of maximizing revenue for a provider \cite{Buchbinder_2007,Blum_2006,Hajiaghayi_2007,Zhou_2008,devanur2009adwords}. We here focus our attention on a few select papers that closely align with the present work.

The initial work on nonlinear \textsc{MaxMin} objective was focused on the \emph{machine covering}, where the goal is to design an algorithm that maximizes the minimum job duration distributed across a set of machines \cite{Azar_1998}. This scheduling problem was first studied in the \emph{semi-online} setting (where the optimal solution value is known by the algorithm) by Ebelendr \cite{Ebenlendr_2005} where a deterministic algorithm was found to give a constant competitive ratio for an idealized input stream. Further work on this problem devised various relaxations of the problem setting such as allowing for some reordering in the allocation process \cite{Epstein_2011}, restricting the number of agents \cite{he2005optimal,tan2006semi,wu2014optimal}, as well as migration of jobs after assignment \cite{chen2011line}. These works in general only consider worst case guarantees, with the literature on the more relaxed input settings being limited.

Most similar to our result is that of Gollapudi and Panigrahi \cite{Gollapudi_2014}, which considers the online \textsc{MaxMin} problem subject to budgeting constraints among other fairness objectives. The work presents a nearly optimal $(1-\ve)$-competitive algorithm for the i.i.d. input setting by means of a weighted greedy algorithm to account for the varying budgets of participating agents. Despite these positive results, the authors do not extend their results to the more complex and practical \emph{random order model}, a novel result presented in the our paper. Furthermore, while the authors make the assumption that the optimal offline solution is lower bounded as $\Omega \left(\frac{\log n}{\ve} \right)$ they do not provide a proof on the necessity of such an assumption, a point that we make clear in the present work. We furthermore note that, when budgeting constraints are removed, the author's algorithm is simply greedy with respect to a negative exponential. This further validates the algorithmic approach we take to the online Santa Claus problem.

Additionally, the online \textsc{MaxMin} was examined by Kawase and Sumita \cite{Kawase_2021}. The authors here demonstrate a $(1-\ve)$ competitive ratio in the unknown i.i.d. setting as well as various hardness results on the adversarial input model. While the authors achieve this result with a unique multiplicative weights update approach in line with \cite{Devanur_2011}, they ultimately do not provide an extension beyond the results presented in \cite{Gollapudi_2014}. Specifically, the authors reiterate that an important extension would be to assume a random-order input model while noting that such results can likely only be achieved by proving a lower bound on the offline hardness of the input instance. Our paper proceeds by presenting exactly these results and achieves this by a simple approximately greedy approach. \todo{maybe not necessary to discuss this preprint, but their lack of novel results do further bolster ours?}

Closely related to our problem is that of online bin packing, where the objective is to place the arriving items are to be placed in bins that have some fixed limited capacity such that the items are fairly distributed without exceeding these capacities \cite{buchbinder2009online,buchbinder2005online,feldman2010online}. This problem has been extensively studied under all input models, with near optimal results being obtained for the random order and i.i.d. setting subject to constraints on the input size \cite{Agrawal_2014} \todo{cite more}. In particular, \cite{Agrawal_2014} proves that, in the random order model, an algorithm can achieve a competitive ratio of $1-\ve$ if and only if the input packing constraints exceed $\Omega \left( \frac{\log n}{\ve^2} \right)$. This result is derived by a careful worse-case example construction, a method that we closely follow in the construction of our impossibility results for the current problem, though we achieve the looser $\Omega \left( \frac{\log n}{\ve} \right)$ bound. The discrepancy between these two results may be of independent interest to the reader.

A companion result to our work is that of Molinaro \cite{Molinaro_2017} which studies the dual ``load balancing'' (or makespan) problem, building upon prior results for the experts approach \cite{Gupta_2014}. In this setting, the algorithm instead attempts to minimize the maximal load distributed to any agent in the system for equitable distribution. This work examines algorithms that work well in both the adversarial and random-order model, balancing the hardness of the two distinct input streams. In achieving their results, the authors relax the maximum function to a general $L^p$ norm and analyze the problem as it depends on the parameter $p$. We here extend their results by emulating the proof technique for the \emph{concave} objective function of a smoothed minimum. As such, we are examining their results for the $p = \infty$ setting while inverting the objective function. As we will demonstrate in the competitive ratio analysis, our results are effectively the dual compliment to the prior work. While in general minimization and maximization problem solutions do not align, we demonstrate that in this problem instance the two align well. We additionally note that while the work of Molinaro does briefly mention that their results improve with some assumption on the optimal offline solution, they fail to provide any lower bounding results. We here emphasize the crucial nature of such a result, and prove the lower bounding result necessary to achieve the desire near optimal competitive ratios.
}



==> TrashFiles/lower_ms.tex <==
% \subsection{High Probability Proof}
\begin{theorem} \label{thm.lb}
	For any $\varepsilon \in (0,1)$, if a randomized algorithm for the online Santa Claus problem with random order input satisfies $$\textsc{ALG} \geq (1-\varepsilon) \cdot \textsc{OPT}$$ then $\textsc{OPT} \geq C \cdot \frac{\ln n}{\varepsilon^2}$ for some (absolute) constant $C > 0$.
\end{theorem}
\noindent We first note that the above theorem implies further implies that any algorithm that achieves the $(1-\varepsilon)$-competitive ratio must necessarily make \emph{at most} $\varepsilon \cdot \textsc{OPT}$ total mistakes in the allocation procedure. We prove the theorem by providing a hard input instance such that, in order to gauruntee the upper bound on the number of mistakes, we must have $\textsc{OPT} = \Omega \left(\frac{\log n}{\varepsilon^2}\right)$. 

We utilize the following adversarial construction: there are $n$ agents, each of which contributes $k$ items divided into two types
\begin{enumerate}
	\item ``Public'' items - have a valuation of 1 for every agent
	\item ``Private'' items - have a value of 1 to that agent and 0 for all others
\end{enumerate}
The number of private items to agent $i$ is denoted $s_i$ and is drawn from the distribution $s_i \sim Binom(k,p)$ where $p$ is to be defined later. An optimal solution is to assign each agent's $k$ items to themselves, giving $\textsc{OPT} = k$. The adversary further selects the probability $p$, to be defined later.

We first prove a lower bound on the number of private items for any agent and thus the minimal guaranteed allocation value.

\begin{lemma} \label{lem.priv}
	With high probability, the number of private items specific to any agent $i$ is at least $kp - \sqrt{4kp(1-p)\log n}$.
\end{lemma}
\begin{proof}
	For our binomial distribution on public items, $r_i \sim Binom(k,1-p)$ we have
$$\Pr \left( \max_i r_i \geq k(1-p) + \sqrt{2kp(1-p) (\log n + t)} \right) \leq e^{-t}$$
Setting $t = \log n$ gives us the succinct
$$\Pr \left( \max_i r_i \geq k(1-p) + \sqrt{4kp(1-p)\log n} \right) \leq \frac{1}{n}$$
Lastly, noting that the number of \emph{private} items is simply $k$ minus the above quantity we have that $$\Pr \left( \min_i s_i \leq kp - \sqrt{4kp(1-p)\log n} \right) \leq \frac{1}{n}$$
and therefore, the probability that lower  bound holds is $1-1/n$. % \todo{cite this Probability bound (or just prove it directly from normal approximation)}

\end{proof}

We now compensate for the number of public items such an agent with the minimal number of private items can expect to receive in the online allocation procedure. Each agent contributes $r_i \sim Binom(k,1-p)$ public items to the online stream, and by nature of the randomized algorithm can expect to receive any of the $\sum_i r_i$ public items with probability $\frac{1}{n}$. Combining these facts we prove the following probabilistic result on the distribution of these public items.

\begin{lemma} \label{lem.pub}
	With high probability, each agent will receive at least $k(1-p) - \sqrt{6(1-p)k\log n}$ public items.
\end{lemma}
\begin{proof}
	If the \emph{total} number of public items is $R \sim Binom(nk, 1-p)$, then the number of items allocated to the $i$-th agent is distributed as $R_i \sim Binom(nk, \frac{1-p}{n})$ essentially stating that over the total number of public items, each is allocated to the $i$-th agent with probability $\frac{1}{n}$. Moreover, each of the $nk$ items has probability $\frac{1-p}{n}$ probability of being allocated to $i$.
	
	We now invoke the Chernoff bound to demonstrate that, since the expected number of public items given to the $i$-th agent is $\frac{1-p}{n} \cdot nk = k(1-p)$, the probability of $R_i$ being small is
	$$\Pr \left( R_i \leq (1-\delta)k(1-p) \right) \leq e^{-\delta^2(1-p)k/3}$$
	We now take the union bound over all $i \in [n]$ to conclude that the probability that \emph{any} agent is allocated less than $(1-\delta)(1-p)k$ public items is at most $ne^{-\delta^2(1-p)k/3}$.
	
	Now setting $\delta = \sqrt{\frac{6 \log n}{(1-p)k}}$ gives us that the probability of any agent being allocated less than $\left(1-\sqrt{\frac{6 \log n}{(1-p)k}}\right)(1-p)k$ public items is at most $\frac{1}{n}$. Therefore, with probability $1-\frac{1}{n}$ all agents are allocated at least $k(1-p) - \sqrt{6(1-p)k\log n}$.
\end{proof}

We now combine the two lemmas to prove conditions on the optimal solution value such that a randomized algorithm can produce a near optimal solution.

\begin{proof}[Proof of Theorem \ref{thm.lb}]
	Taking a union bound over the two events depicted in Lemmas \ref{lem.priv} and \ref{lem.pub} we have that, with probability at least $1-\frac{2}{n}$, every agent $i$ must be allocated at least
	\begin{align*}
		\left(kp - \sqrt{4kp(1-p)\log n}\right) +  \left(k(1-p) - \sqrt{6(1-p)k\log n}\right) \\
		= k - \sqrt{k (1-p) \log n} \cdot (\sqrt{4p} + \sqrt{6})
	\end{align*}
	Therefore, in order to have at least a $(1 - \varepsilon)k$ solution, it must be the case that $$k - \sqrt{k (1-p) \log n} \cdot (\sqrt{4p} + \sqrt{6}) \geq (1-\varepsilon)\textsc{OPT}$$
	Simplifying gives us the condition $$k > 4\sqrt{\frac{6(1-p)^2 p \log^2 n}{\varepsilon^4}} - \frac{2(2p^2 + p - 3)\log n}{\varepsilon^2}$$
	which an adversary can maximize by selecting $p = \mathcal{O}(1)$ appropriately to give $$k = \Omega\left( \frac{\log n}{\varepsilon^2} \right)$$
	Thus, we have that $\textsc{OPT} = k = \Omega\left( \frac{\log n}{\varepsilon^2} \right)$ completing the result.
\end{proof}


==> TrashFiles/nov15_notes.tex <==
\begin{document}
\section{Summary}
List of Current Results:
\begin{enumerate}
    \item Lower bound on deterministic algorithm under adversarial input
    \item Lower bound on random algorithm under adversarial input
    \item $(1-\epsilon)$ competitive ratio under IID input with known \opt{} and \emph{integral} allocation
\end{enumerate}
List of Results to Obtain
\begin{enumerate}
    \item $(1-\epsilon)$ competitive ratio under IID input with \emph{unknown} \opt{} and integral allocation
    \item Some competitive ratio under random order input (integral allocation)
\end{enumerate}
\section{Problem Defintion and Preliminaries}
We seek to allocate a set of $m$ indivisible goods ($\mathcal{M} = [m]$) equitably across $n$ agents ($\mathcal{N} = [n]$), where $n \leq m$. In particular, we define a \emph{fair allocation} as one that maximizes the minimal bundle value to any agent (the so-called \textsc{MaxMin} problem). Formally, let $v_{ij}$ denote the value of good $j$ to agent $i$ and let $\mathcal{S}_i$ denote the subset of items allocated to agent $i$. The problem described above is thus $$\max \min_i \sum_{j \in \mathcal{S}_i} v_{ij}$$ We furthermore reduce the problem to that of the \emph{Santa Claus problem} with unit valued goods: $v_{ij} \in \{0,1\}$ for all $j \in \mathcal{M}$.

We examine the \textsc{MaxMin} problem from the online setting, where goods to be allocated arrive one at a time and need to be permanently assigned to an agent upon arrival. We will examine this problem under both the IID, random-order and adversarial frameworks. We assess the quality of our algorithms by their \emph{competitive ratio}, or the ratio of our online algorithms solution to that of the optimal \emph{offline} solution (denoted \opt{}). More formally, let $\mathcal{I}$ denote an arbitrary problem instance and \textsc{Alg} denote the solution value output by the designed online algorithm, then the competitive ratio is at least $c$ when, for constant $b \geq 0$: $$\textsc{alg}(\mathcal{I}) \geq c \cdot \opt{}(\mathcal{I}) - b$$

\section{Adversarial Counterexamples}
We here present lower bounds on the problem context under an adversarial input model. This is the setting in which an adversary presents a worst-case input by selecting both the item values for each agent and the order in which items arrive (thus constructing the difficult allocation problem istances). Our first result of this kind is the following theorem.

%\begin{theorem} \label{thm.simple_counter}
 %   There is no randomized algorithm that obtains a competitive ratio better than $\frac{1}{n}$ for the online \textsc{MaxMin} problem.
%\end{theorem}

\begin{theorem} \label{thm.determin_bound}
    The competitive ratio of any deterministic algorithm is zero under the adversarial arrival input model.
\end{theorem}
\begin{proof}
    Let \textsc{alg} be a fixed deterministic algorithm and assume that the adversary picks the first item to have value 1 for all $n$ agents. Assume \textsc{alg} allocates this item to the first agent without loss of generality. Now assume that for the following $n-1$ items, the adversary presents items of value 1 to all agents but the $n$-th agent. Then regardless of how \textsc{alg} assigns these items, $v_n(\mathcal{S}_n) = 0$ whereas the optimal offline value is \opt{} $= 1$. Thus, the competitive ratio is 0.
\end{proof}

\begin{comment}
\begin{theorem} \label{thm.random_bound}
    The competitive ratio of any randomized algorithm is at most $\frac{1}{n}$ under the adversarial arrival input model.
\end{theorem}
\begin{proof}
    
\end{proof}
\begin{proof}
    Let \textsc{alg} be any randomized algorithm (where \textsc{alg} $= \min_i \sum_{j \in \mathcal{S}_i} v_{ij}$) and let $\pi$ be a permutation of $[n]$ chosen uniformly at random. Assume the adversarial input sequence consists of $n$ items with values defined as 
    \begin{align*}
        v_{ij} = 
    \begin{cases} 
      0 & \text{if } i \in \{\pi(1), ..., \pi(j-1)\} \\
      1 & \text{if } i \in \{\pi(j), ..., \pi(n)\}
    \end{cases}
    \end{align*}
    For this input, \opt{} $=1$ if and only if item $j$ is assigned to agent $\pi(j)$ and \opt{} $=0$ otherwise. The probability that the $j$-th item is allocated to agent $\pi(j)$ is at most $\frac{1}{n-(j-1)}$. Therefore, the probability of \textsc{alg} yielding a nonzero value is given by
    \begin{align*}
        \mathbb{P}[\textsc{alg} = 1] &\leq \prod_{j=1}^n \frac{1}{n-(j-1)} \\
        &= \frac{1}{n!}
    \end{align*}
    Thus, we have $\mathbb{E}[\textsc{alg}] \leq \frac{1}{n!} \cdot 1 = \frac{1}{n!}$, giving us the result.
\end{proof}
\end{comment}

\begin{comment}
Let $\mathcal{A}$ denote the set of deterministic algorithms and $\mathcal{X}$ the set of permutations of the inputs to an online algorithm, where item values are selected adversarially. Furthermore, let $r(a,x)$ be the reward that algorithm $a$ achieves on instance $x$. To prove this result we utilize the following result from Yao\footnote{citation}
\begin{lemma}[Yao's Minimax Principle]
    Let $\mathcal{A}$ be a random variable with values in $A$ and let $X$ be a random variable with values in $\mathcal{X}$. Then, $$\min_{x \in \mathcal{X}} \mathbb{E}[r(\mathcal{A},x)] \leq \max_{a \in \mathcal{A}} \mathbb{E}[r(a,\mathcal{X})]$$
\end{lemma}

We now prove the theorem.
\begin{proof}
    Assume we have $n$ items and $n$ agents. An adversary selects an input such that item $j \in \mathcal{M}$ has value $v_{jj}) = 1$ and $v_{ij} = 0$ for all $i \neq j$ and $j \in [n-1]$. We call these items ``private" to a specific agent. Lastly, item $n$ has value 1 for all $n$ agents. We call this item a ``public" good. In the offline problem, we simply assign each private item to the corresponding private agent and the public good to the $n$-th agent, giving a \textsc{MaxMin}$=1$ (our \opt{} value). Let $\mathcal{X}$ denote the set of permutations of this stream of $n$ items and let $\mathcal{A}$ denote the set of algorithms which assign arriving items to agents with a nonzero value, breaking ties randomly. We furthermore define $p(a,x) = 1$ for $x \in \mathcal{X}, a \in \mathcal{A}$ if the algorithm achieves a \textsc{MaxMin} value of 1 (all agents receive an item). We calculate
    $$\max_{a \in \mathcal{A}} \mathbb{E}[r(a,\mathcal{X})] = \frac{1}{n}$$
    and by Yao's principle we have the following result $$\min_{x \in \mathcal{X}} \mathbb{E}[r(\mathcal{A},x)] \leq \frac{1}{n}$$ Lastly, comparing this upperbound to \opt{} gives us the competitive ratio result:
    $$\frac{\min_{x \in \mathcal{X}} \mathbb{E}[r(\mathcal{A},x)]}{\opt{}} \leq \frac{1}{n}$$
\end{proof}

Building on this simple counterexample, we are able to prove a lower bound on the value of \textsc{Opt}.

\begin{theorem} \label{thm.boosted_counter}
    \opt{} has a lower bound of $\log n$. \todo{Need to properly state and formalize this result, but I think the intuition is currently there. Revisit.}
\end{theorem}
\begin{proof}
    Assume we have $n$ agents and $n$ item \emph{types} which are broken down in the following way: items $n_i$ for $i \in [n-1]$ are ``private" meaning they have value 1 to their corresponding agent $i$ and 0 for the others ($j \neq i$). Lastly, the $n$-th item type is ``public" meaning it has a value of 1 for all agents. Further assume we have $k$ of each item type, giving us $nk$ total items. 
    
    In the offline scenario, each agent receives exactly $k$ items of their specific type (where the agent without a private good must receive all the public goods) to achieve $\textsc{Opt} = k$. Analysis of the error in our online setting is measured in terms of how many of the public goods are assigned \emph{improperly}, since the private goods will always be correctly assigned (as they can only be allocated to their corresponding agent). 
    
    In the case where items arrive in a random online fashion, we first consider sampling from the items \emph{with} replacement to motivate the analysis of the real problem \emph{without} replacement.
    
    When sampling with replacement, we essentially have $k \rightarrow \infty$. Let $T$ be the number of samples required to obtain one of each item type, and let $t_i$ be the time required to see an item of type $i$. Thus $$T = t_1 + t_2 + ... + t_n$$ and the probability of seeing a unique item is $$p_i = \frac{n-(i-1)}{n}$$ We furthermore have that $t_i$ has a geometric distribution with expectation $\frac{1}{p_i}$. Now we can derive 
    \begin{align*}
        \mathbb{E}[T] &= \mathbb{E}[t_1 + ... t_n] \\
        &= \mathbb{E}[t_1] + ... \mathbb{E}[t_n] \\
        &= \frac{1}{p_1} + ... + \frac{1}{p_n} \\
        &= n \left( \frac{1}{1} + \frac{1}{2} + ... + \frac{1}{n} \right) \\
        &= n \cdot H_n = \Theta(n \log n)
    \end{align*}
    where $H_n$ is the $n$-th Harmonic number. 
    
    As a result of the above, in the case of $k \gg \log n$ we know that $T \approx n \log n$ with high probability. If we instead consider the case where $k \ll \log n$ (or moreso $\lim_{n \rightarrow \infty}\frac{k}{\log n} = 0$), then each of the $nk$ balls is drawn with probability $$1 - \left(1 - \frac{1}{nk}\right)^t$$ on the $t$-th sample. Let $D$ denote the number of \emph{unique} items seen thus far. We have that the expectation of $D$ is $$\mathbb{E}[D] = nk \cdot \left(1 - \left(1 - \frac{1}{nk}\right)^t\right) \approx nk \cdot (1 - e^{-t/nk})$$
    where the approximation holds for $n$ large enough. We now let $t = \alpha \cdot n \log n$ for some $\gamma \in (0,1]$, and we can write the expectation as 
    \begin{align*}
        \mathbb{E}[D] &= nk \cdot \left(1 - \left(1 - e^{-c \log n / k}\right)\right) \approx nk
    \end{align*}
    Therefore, if $k$ is growing faster than $\log n$, we have that approximately $n \log n$ draws to see one of each type, and in the converse case, we will have $nk$.
\end{proof}
\end{comment}

\section{IID Model}
\subsection{Preliminaries} We assume that the probability an item has value 1 to agent $i$ is $p_i$ (and value 0 with probability $1-p_i$) where $p_i$ is unknown.
\vspace{2.5mm}\\
For future reference, we can formalize the \textsc{MaxMin} problem with the following LP, where $x_{ij}$ denotes the fraction of item $j$ assigned to agent $i$:
\begin{gather*}
\max \lambda \\
\begin{aligned}
\textup{s.t.}\quad &\forall i \in \mathcal{N} \quad \sum_j v_{ij} \cdot x_{ij}  \geq  \lambda \\
            &\forall j \in \mathcal{M} \quad \sum_i x_{ij} \leq 1
\end{aligned}
\end{gather*}
We can additionally define the ``expected instance" LP (to be used in Section 4.2) as
\begin{gather*}
\max \lambda \\
\begin{aligned}
\textup{s.t.}\quad &\forall i \in \mathcal{N} \quad p_i \sum_j v_{ij} \cdot x_{ij}  \geq  \frac{\lambda}{m} \\
            &\forall j \in \mathcal{M} \quad \sum_i x_{ij} \leq 1
\end{aligned}
\end{gather*}
Of note, we will only use the above LPs in \emph{analyzing} our algorithm\footnote{The analysis relies on knowing the value of $m$ as well, which is not necessarily a given.}. 
\subsection{Potential-Based Greedy Algorithm}
Let \opt{} denote the maximal value achieved in the offline setting to the \textsc{MaxMin} problem. We will here assume that the value of \opt{} is known (or can be estimated with minimal reduction in approximate value). Our algorithm works by greedily assigning items according to an exponential reward function. We define the following potential function $$\phi(k) = \left(\frac{\alpha \ln n}{\opt{}}\right) exp\left(- \frac{\alpha \ln n}{\opt{}} \cdot k \right)$$ where $\alpha$ is a constant we will fix later. We additionally define $$\overline{\Phi}(k) = \int_{j=k}^{\infty} \phi(j) dj$$
We can thus define the ``remaining reward" for agent $i$ at any stage of the algorithm by $\overline{\Phi}_i = \overline{\Phi}(c_i)$ where $c_i$ is the current coverage of agent $i$, and the \emph{overall} remaining reward is $\overline{\bold{\Phi}} = \sum_{i \in D} \overline{\Phi}_i$.
\vspace{2.5mm}\\
Let $j$ be the current request in the input stream. If the fractional coverage is $c_i$ for some agent $i$, then the reward $r_{ij}$ of allocating $j$ to $i$ is \emph{decrease} in the value of $\overline{\bold{\Phi}}$: $$r_{ij} = \int_{k=c_i}^{c_i + v_{ij}} \phi(k) dk$$ The \textsc{MaxMin} algorithm greedily assigns impressions based on this reward function.
 We here derive the competitive ratio of the above greedy approach where we assume the item values are drawn from an unknown distribution. 
%In the same vein as the paper, we assume that $$\opt{} = \alpha \ln n \geq \frac{\ln n}{2\epsilon}$$ or moreso $\opt{} = \Omega \left(\frac{\log n}{\epsilon}\right)$.
\begin{theorem} \label{thm.reward_comp}
    For any $\epsilon > 0$, the competitive ratio of the above algorithm for the \textsc{MaxMin} problem is $1-\epsilon$, assuming $\opt{} = \Omega \left(\frac{\log n}{\epsilon}\right)$.
\end{theorem}
\noindent  We first make the definition $\opt{} = \alpha \ln n \geq \frac{\ln n}{2\epsilon}$ in accordance with the $\opt{} = \Omega \left(\frac{\log n}{\epsilon}\right)$ assumption. In proving the theorem, we first need to assemble some lemmas which will combine to yield the result.
\begin{lemma} \label{lemma.LPbound}
    At any stage of the algorithm, the expected decrease in $\overline{\bold{\Phi}}$ for the next arriving impression is at least $(1-\epsilon)\frac{\alpha \ln n}{m}\overline{\bold{\Phi}}$.
\end{lemma}
\begin{proof}
    In proving this lemma, we revisit the expected LP formulation of the problem. We compare the decrease in potential of our algorithm to that of the hypothetical fractional algorithm which exactly follows the LP assignment. Our algorithm maximizes the decrease in potential at every step, and therefore any lower bound on the expected decrease in the LP-based algorithm is \emph{also a lower bound for our algorithm}. We reiterate that our algorithm yields an integral solution and cannot use the above LP.
\begin{gather*}
\begin{aligned}
    &\forall i \in \mathcal{N} \quad p \sum_j v_{ij} \cdot x_{ij}  \geq  \frac{\lambda}{m} \\
    &\forall j \in \mathcal{M} \quad \sum_i x_{ij} \leq 1
\end{aligned}
\end{gather*}
The first constraint ensures that each agent is assigned at least the optimal amount in expectation and the second ensures that impressions are allocated at most in their entirety. The expected decrease in $\overline{\bold{\Phi}}$ for an algorithm which fractionally assigns impression $j$ with probability $x_{ij}$ at any stage is 
\begin{gather*}
    \sum_i \sum_j p \cdot x_{ij} \int_{k=c_i}^{c_i + v_{ij}} \phi(k) dk \\
    = \sum_i \sum_j p \cdot x_{ij} \cdot \phi(c_i) \cdot v_{ij} \cdot \left( \frac{\opt{}}{\alpha v_{ij} \ln n} \right)\left(1 - e^{\frac{- \alpha v_{ij} \ln n}{\opt{}}}\right)
\end{gather*}
Using the fact that $\frac{1-e^{-x}}{x} \geq 1 - x/2$, we thus obtain
\begin{gather}
    \geq \sum_i \sum_j p \cdot x_{ij} \cdot \phi(c_i) \cdot v_{ij} \cdot \left( 1 - \frac{\alpha v_{ij} \ln n}{2 \opt{}}\right) \\
    \geq \sum_i \sum_j p \cdot x_{ij} \cdot \phi(c_i) \cdot v_{ij} \cdot (1-\epsilon)
\end{gather}
where the second inequality comes from $v_{ij} \leq 1$ and the assumed bound on \opt{}. Finally, rearranging the terms and utilizing the bound from the expected LP gives us
\begin{gather*}
    \geq (1-\epsilon) \sum_i \frac{\phi(c_i) \opt{}}{m} = (1-\epsilon)\frac{\alpha \ln n}{m} \overline{\bold{\Phi}}
\end{gather*}
\end{proof}
We now prove the following lemma that demonstrates how Lemma \ref{lemma.LPbound} gives us the proof of Theorem \ref{thm.reward_comp}. The above lemma implies that the value of $\overline{\bold{\Phi}}$ decreases to at most $$\left(1 - \left(1-\epsilon\right) \frac{\alpha \ln n}{m} \right) \cdot \overline{\bold{\Phi}} \leq n^{-(1-\epsilon)\frac{\alpha}{m}} \cdot \overline{\bold{\Phi}}$$, since $1-x \leq e^{-x}$. Using this repeatedly over $m$ requests, we get the expected value of $\overline{\bold{\Phi}} \leq n^{-(1-\epsilon)} \overline{\bold{\Phi}}_0$ where $\overline{\bold{\Phi}}_0$ is the initial value of the remaining reward function. Lastly, noting that $$\overline{\bold{\Phi}}_0 = \sum_i \overline{\Phi}(0) = \sum_i 1 = n$$ we have that the expected value when the algorithm terminates is at most $n^{1-(1-\epsilon)}$. We can now prove Theorem \ref{thm.reward_comp} by contradiction.
\begin{proof}
    Assume for some agent $i_{\min}$ that the fraction coverage $c_{i_{\min}} < (1-\epsilon) \opt{}$ at the algorithms termination. Then,
    $$\overline{\bold{\Phi}} = \sum_i \overline{\Phi}_i \geq n \cdot \overline{\Phi}_{i_{\min}} = n \cdot n^{-\frac{c_{i_{\min}}}{\opt{}}} > n \cdot n^{-(1-\epsilon)} = n^{1-(1-\epsilon)}$$ which contradicts the expected maximal value of $\overline{\bold{\Phi}}$ at the end of the algorithm. Therefore, each $c_i \geq (1-\epsilon) \opt{}$.
\end{proof}
\begin{comment}
\todo{Formalize result below when opt is small}
\subsection{Constraining OPT} We can additionally run the above algorithm with $\opt{}^\epsilon = \max \{\opt{}, \frac{\log n}{\epsilon^2} \}$ without placing an assumption on the value of \opt{}, giving us an additional additive factor for the approximation. This will give us an algorithmic guarantee of
\begin{align*}
    \textsc{alg} \geq (1-\epsilon) \opt{}^\epsilon > (1-\epsilon)\opt{} - \frac{\log n}{\epsilon^2}
\end{align*}
\end{comment}

\newpage

\begin{comment}
\section{Random Order Model Notes} 
We now work under the \emph{random order model} (ROM): the setting where an adversary selects the set $\mathcal{I}$ of items but not the sequence. The items of this set are then presented to the algorithm in a uniformly random order. Formally, given a set $\mathcal{I} = \{s_1, s_2, ... s_m \}$ of $m = |\mathcal{I}|$ items, we imagine drawing a uniform random permutation $\sigma$ of $\{1,...,m\}$ and then the input sequence to our algorithm is $s_{\sigma(1)}, s_{\sigma(2)}, ..., s_{\sigma(m)}$. The ROM is a generalization of the IID model and can be seen as sampling \emph{without} replacement versus with replacement. As such, we expect the competitive factor under ROM to be weaker but close to the $(1-\epsilon)$ result prove above.

\subsection{Greedy-Potential Algorithm} Can we prove a $(1-\epsilon)$ competitive factor for the above algorithm?

\subsection{OCP Algorithm} Can we prove a $(1-\epsilon)$ competitive factor using the OCP method? To implement the Agrawal and Devanur method we need a concave ($L$-Lipschitz) objective function $f$ and a optimal estimated parameter $Z$ which captures the tradeoff between objective value and distance to the \emph{convex} constraint set $S$. The logical implementation would be as follows:
\begin{enumerate}
    \item $f(x_1,...,x_n) = \frac{-1}{\epsilon} \log\left( e^{\epsilon x_1} + ... + e^{\epsilon x_n} \right) \approx \min \{x_1,...,x_n\}$ as our concave objective function
    \item The above is $1$-Lipschitz continuous (so $L = 1$).
    \item Lastly, we need to pick a $Z$ parameter such that the following holds: Let $\opt{}^{\delta}$ denote the optimal value of the offline problem that minimizes $f(\frac{1}{T} \sum_t \bold{x}_t)$ with the feasibility constraint relaxed to $d(\frac{1}{T}\sum_t \bold{x}_t,S) \leq \delta$. Then we need to pick a $Z \geq 0$ such that for all $\delta \geq 0$, $$\opt{}^{\delta} \leq \opt{} + Z\delta$$
\end{enumerate}
Define  avg-regret$(T) = \opt{} - f(\bold{x}_{avg})$ then we have the following theorem due to Agrawal and Devanur
\begin{theorem}
    There is an algorithm (see paper) that achieves the following regret guarantees for the Online Stochastic Convex Programming problem in the random order model.
    \begin{align*}
        \mathbb{E}[\text{avg-regret}(T)] = (Z+L) \cdot O \left( \sqrt{\frac{C}{T}}\right)
    \end{align*}
    where $C$ depends on the norm used for defining distance. For Euclidean norm, $C = n \log(n)$. For $L_\infty$ norm, $C = \log(n)$. The parameter $Z$ captures the tradeoff between objective and constraints for the problem, its value is problem-dependent. $L$ is the Lipschitz constant for $f$ w.r.t. the same norm as used to measure distance.
\end{theorem}
Thus, in our context, depending on our estimate for $Z$ we have $$\mathbb{E}[\text{avg-regret}(T)] = (Z+1) \cdot O \left( \sqrt{\frac{n \log n}{T}}\right)$$
How do we adequately pick $Z$ and subsequently carry out the proof as for the online packing/covering LPs in order to convert the regret guarantee to a competitive ratio?
\end{comment}

\end{document}

==> TrashFiles/other_notes.tex <==
\begin{document}
\section{Discussed / Expected Results}
\begin{enumerate}[leftmargin=*]
    \item Simple counterexample in the adversarial input case (Theorem \ref{thm.simple_counter})
    \item ``Boosted" adversarial counterexample to assert that \opt{} $= \Omega(\log n)$. (Theorem \ref{thm.boosted_counter})
    \item Online algorithm with $(1 - \epsilon)\opt{}$ approx. using reward potential function from Gollapudi, Panigrahi 2014. (Theorem \ref{thm.reward_comp})
    \item Online algorithm with $(1 - \epsilon)\opt{}$ approx. using Devanur/Jain/Sivan/Wilkens paper method.
    \item Online algorithm with $(1 - \epsilon)\opt{} + \frac{\log n}{\epsilon^2}$ approx. using Agrawal/Devanur paper method.
\end{enumerate}

\section{Adversarial Counterexamples}
\begin{theorem} \label{thm.simple_counter}
    There is no randomized algorithm that obtains a competitive ratio better than $\frac{1}{n}$ for the online \textsc{MaxMin} problem.
\end{theorem}
\begin{proof}
    Assume we have $n$ items and $n$ agents. An adversary selects an input such that item $x_j$ has value $v_j(x_j) = 1$ and $v_i(x_j) = 0$ for all $i \neq j$ and $j \in [n-1]$. We call these items ``private" to a specific agent. Lastly, item $x_n$ has value 1 for all $n$ agents. We call this item a ``public" good. Let $\mathcal{X}$ denote the set of permutations of this stream of $n$ items and let $\mathcal{A}$ denote the set of deterministic algorithms where each arriving item is assigned to a predefined agent in the sequence from 1 to $n$. We furthermore define $p(a,x) = 1$ for $x \in \mathcal{X}, a \in \mathcal{A}$ if the algorithm achieves a coverage of 1 for all agents. We calculate
    $$\max_{a \in \mathcal{A}} \mathbb{E}[p(a,\mathcal{X})] = \frac{1}{n}$$
    and by Yao's principle we have the result.
\end{proof}

\begin{theorem} \label{thm.boosted_counter}
    \opt{} has a lower bound of $\log n$. \todo{Need to properly state and formalize this result, but I think the intuition is currently there. Revisit.}
\end{theorem}
\begin{proof}
    Assume we have $n$ agents and $n$ item types which are broken down in the following way: items $n_i$ for $i \in [n-1]$ are ``private" meaning they have value 1 to their corresponding agent $i$ and 0 for the others ($j \neq i$). Lastly, the $n$-th item type is ``public" meaning it has a value of 1 for all agents. Further assume we have $k$ of each item type, giving us $nk$ total items. In the offline scenario, each agent receives exactly $k$ items of their specific type (where the agent without a private good must receive all the public goods). Analysis of the error in our online setting is measured in terms of how many of the public goods are assigned improperly, since the private goods will always be correct assigned. If we consider the case where items arrive in a random online fashion, we first consider sampling from the items \emph{with} replacement to motivate the analysis of the real problem \emph{without} replacement.
    
    When sampling with replacement we have the well-known ``coupon collector" problem. Consider the arrival of items until one of each type is seen. Let $M$ be the number of items drawn thus far, and $D$ be the number of \emph{distinct} items. We know that $M$ will be close to $n \log n$ with high probability (assuming $k \gg \log n$). If we consider the case where $k \ll \log n$ (or moreso $\lim_{n \rightarrow \infty}\frac{k}{\log n} = 0$), then each of the $nk$ balls is drawn with probability $$1 - (1 - \frac{1}{nk})^m$$ on drawing $m$. Thus, the expectation of $D$ is $$\mathbb{E}[D] = nk \cdot \left(1 - \left(1 - \frac{1}{nk}\right)^m\right)$$
    Informally, for $n$ large enough, this is approximately $nk \cdot \left(1-e^{-m/nk}\right)$. Now let $m = c \cdot n \log n$ for some $c \in (0,1]$, and we can write the expectation as 
    $$\mathbb{E}[D] = nk \cdot \left(1 - \left(1 - e^{-c \log n / k}\right)\right) \approx n \cdot k$$
    where the approximation comes from our assumption on the ratio of $k$ to $\log n$. So if $k$ is growing faster than $\log n$, we have that approximately $n \log n$ draws to see one of each type, and in the converse case, we will have $nk$.
    \todo{formalize and finish this proof.}
\end{proof}

\section{Online Algorithms}
\subsection{Preliminaries} We assume that each impression $j \in \mathcal{J}$ (where $|\mathcal{J}| = m$) has value to an agent $i \in D$ of 0 or 1, denoted by $v_{ij} \in \{0,1\}$. The item valuation profiles $\bold{v}_j$ are selected by an adversary and presented in a random order, with the probability that $v_{ij} = 1$ denoted by $p_{ij}$. We present the \textsc{MaxMin} problem as attempting to maximize the minimal value given to any agent: $\max \min_{i \in D} \sum_j v_{ij} \cdot x_{ij}$ where $x_{ij}$ is the (fractional) allocation of impression $j$ to $i$.
\vspace{2.5mm}\\
For future reference, we can formalize the \textsc{MaxMin} problem with the following LP:
\begin{gather*}
\max \lambda \\
\begin{aligned}
\textup{s.t.}\quad &\forall i \in D \quad \sum_j v_{ij} \cdot x_{ij}  \geq  \lambda \\
            &\forall j \in \mathcal{J} \quad \sum_i x_{ij} \leq 1
\end{aligned}
\end{gather*}
We can additionally define the ``expected instance" LP as (to be used in Section 3.3)
\begin{gather*}
\max \lambda \\
\begin{aligned}
\textup{s.t.}\quad &\forall i \in D \quad \sum_j p_{ij} \cdot v_{ij} \cdot x_{ij}  \geq  \frac{\lambda}{m} \\
            &\forall j \in \mathcal{J} \quad \sum_i x_{ij} \leq 1
\end{aligned}
\end{gather*}

\subsection{Gollapudi/Panigrahi Greedy Algorithm} Let \opt{} denote the maximal value achieved in the offline setting to the \textsc{MaxMin} problem. We will here assume that the value of \opt{} is known (or can be estimated with minimal reduction in approximate value) \todo{can we get the same guarantee $+ \frac{\log n}{\epsilon^2}$ factor when \opt{} is not assumed?}. As in the original paper, define the following potential function $$\phi(k) = \left(\frac{\gamma \ln n}{\opt{}}\right) exp\left(- \frac{\gamma \ln n}{\opt{}} \cdot k \right)$$ where $\gamma$ is a constant we will fix later. We additionally define $$\overline{\Phi}(k) = \int_{j=k}^{\infty} \phi(j) dj$$
We can thus define the ``remaining reward" for agent $i$ at any stage of the algorithm by $\overline{\Phi}_i = \overline{\Phi}(c_i)$ where $c_i$ is the current coverage of agent $i$, and the \emph{overall} remaining reward is $\overline{\bold{\Phi}} = \sum_{i \in D} \overline{\Phi}_i$.
\vspace{2.5mm}\\
Let $j$ be the current request in the input stream. If the fractional coverage is $c_i$ for some agent $i$, then the reward $r_{ij}$ of allocating $j$ to $i$ is \emph{decrease} in the value of $\overline{\bold{\Phi}}$: $$r_{ij} = \int_{k=c_i}^{c_i + v_{ij}} \phi(k) dk$$ The \textsc{MaxMin} algorithm simply greedily assigns impressions based on the reward function.

\subsubsection{Analysis of algorithm} We here derive the competitive ratio of the above greedy approach. While the original paper has additional packing constraints (budgets), we need not assume a large enough gap between budgets and bids. However, we do need to assume that the optimal value is large enough. In the same vein as the paper, we assume that $$\opt{} = \gamma \ln n \geq \frac{\ln n}{2\epsilon}$$ or moreso $\opt{} = \Omega \left(\frac{\log n}{\epsilon}\right)$.
\begin{theorem} \label{thm.reward_comp}
    The competitive ratio of the above algorithm for the \textsc{MaxMin} problem is $1-\epsilon$.
\end{theorem}
\noindent In proving this theorem, we first need to assemble some lemmas which will combine to yield the result.
\begin{lemma} \label{lemma.LPbound}
    At any stage of the algorithm, the expected decrease in $\overline{\bold{\Phi}}$ for the next arriving impression is at least $(1-\epsilon)\frac{\gamma \ln n}{m}\overline{\bold{\Phi}}$.
\end{lemma}
\begin{proof}
    In proving this lemma, we revisit the expected LP formulation of the problem. Though our algorithm does not utilize the LP to make assignments, it provides the necessary framework to bound the decrease as desired. \todo{Explain why LP bound holds here.}
\begin{gather*}
\begin{aligned}
    &\forall i \in D \quad \sum_j p_{ij} \cdot v_{ij} \cdot x_{ij}  \geq  \frac{\lambda}{m} \\
    &\forall j \in \mathcal{J} \quad \sum_i x_{ij} \leq 1
\end{aligned}
\end{gather*}
The first constraint ensures that each agent is assigned at least the optimal amount in expectation and the second ensures that impressions are allocated at most in their entirety. The expected decrease in $\overline{\bold{\Phi}}$ for an algorithm which fractionally assigns impression $j$ with probability $x_{ij}$ at any stage is 
\begin{gather*}
    \sum_i \sum_j p_{ij} \cdot x_{ij} \int_{k=c_i}^{c_i + v_{ij}} \phi(k) dk \\
    = \sum_i \sum_j p_{ij} \cdot x_{ij} \cdot \phi(c_i) \cdot v_{ij} \cdot \left( \frac{\opt{}}{\gamma v_{ij} \ln n} \right)\left(1 - e^{\frac{- \gamma v_{ij} \ln n}{\opt{}}}\right)
\end{gather*}
Using the fact that $\frac{1-e^{-x}}{x} \geq 1 - x/2$, we thus obtain
\begin{gather}
    \geq \sum_i \sum_j p_{ij} \cdot x_{ij} \cdot \phi(c_i) \cdot v_{ij} \cdot \left( 1 - \frac{\gamma v_{ij} \ln n}{2 \opt{}}\right) \\
    \geq \sum_i \sum_j p_{ij} \cdot x_{ij} \cdot \phi(c_i) \cdot v_{ij} \cdot (1-\epsilon)
\end{gather}
where the second inequality comes from $v_{ij} \leq 1$ and the assumed bound on \opt{}. Finally, rearranging the terms and utilizing the bound from the expected LP gives us
\begin{gather*}
    \geq (1-\epsilon) \sum_i \frac{\phi(c_i) \opt{}}{m} = (1-\epsilon)\frac{\gamma \ln n}{m} \overline{\bold{\Phi}}
\end{gather*}
\end{proof}
We now prove the following lemma that demonstrates how Lemma \ref{lemma.LPbound} gives us the proof of Theorem \ref{thm.reward_comp}. The above lemma implies that the value of $\overline{\bold{\Phi}}$ decreases to at most $$\left(1 - \left(1-\epsilon\right) \frac{\gamma \ln n}{m} \right) \cdot \overline{\bold{\Phi}} \leq n^{-(1-\epsilon)\frac{\gamma}{m}} \cdot \overline{\bold{\Phi}}$$, since $1-x \leq e^{-x}$. Using this repeatedly over $m$ requests, we get the expected value of $\overline{\bold{\Phi}} \leq n^{-(1-\epsilon)} \overline{\bold{\Phi}}_0$ where $\overline{\bold{\Phi}}_0$ is the initial value of the remaining reward function. Lastly, noting that $$\overline{\bold{\Phi}}_0 = \sum_i \overline{\Phi}(0) = \sum_i 1 = n$$ we have that the expected value when the algorithm terminates is at most $n^{1-(1-\epsilon)}$. We can now prove Theorem \ref{thm.reward_comp} by contradiction.
\begin{proof}
    Assume for some agent $i_{\min}$ that the fraction coverage $c_{i_{\min}} < (1-\epsilon) \opt{}$ at the algorithms termination. Then,
    $$\overline{\bold{\Phi}} = \sum_i \overline{\Phi}_i \geq n \cdot \overline{\Phi}_{i_{\min}} = n \cdot n^{-\frac{c_{i_{\min}}}{\opt{}}} > n \cdot n^{-(1-\epsilon)} = n^{1-(1-\epsilon)}$$ which contradicts the expected maximal value of $\overline{\bold{\Phi}}$ at the end of the algorithm. Therefore, each $c_i \geq (1-\epsilon) \opt{}$.
\end{proof}

\subsection{Devanur/Jain/Sivan/Wilkens Method}

We once again utilize the ``expected instance" LP (reprinted here):
\begin{gather*}
\begin{aligned}
    &\forall i \in D \quad \sum_j p_{ij} \cdot v_{ij} \cdot x_{ij}  \geq  \frac{\lambda}{m} \\
    &\forall j \in \mathcal{J} \quad \sum_i x_{ij} \leq 1
\end{aligned}
\end{gather*}

\subsubsection{Known Distribution} \label{sec.known_dis}
When the distributions are \emph{completely known}, we first compute the expected instance and solve the LP optimally. Denote the optimal solution to this LP by $x_{ij}^*$. Our algorithm $P$ works as follows: when request $j$ arrives, it is assigned to $i$ with probability $x_{ij}^*$. We furthermore analyze a more conservative algorith, which we denote $\tilde{P}$: when request $j$ arrives it is assigned to $i$ with probability $\frac{x_{ij}^*}{1+\epsilon}$ for error parameter $\epsilon$. Let $\tilde{Y}_{t}$ denote the increase in value for time step $t$ for the algorithm $\tilde{P}$. Lastly, note that $\mathbb{E}[\tilde{Y}_t] = \sum_i \sum_j p_{ij} v_{ij} \frac{x_{ij}^*}{1+\epsilon} \geq \frac{\opt{}}{(1+\epsilon)m}$. For $\gamma = O\left( \frac{\epsilon^2}{\log (n/\epsilon)} \right)$ we utilize Chernoff bounds to obtain the following:
\begin{align*}
    \mathbb{P}\left[ \sum_t \tilde{Y}_t \leq \frac{\opt{}}{1+\epsilon}(1-\epsilon)\right] &= \mathbb{P}\left[\frac{\sum_t \tilde{Y}_t}{\gamma \opt{}} \leq \frac{1-\epsilon}{\gamma(1+\epsilon)} \right] \\
    &= \mathbb{P}\left[ (1-\epsilon)^{\frac{\sum_t \tilde{Y}_t}{\gamma \opt{}}} \geq (1-\epsilon)^{\frac{1-\epsilon}{\gamma (1+\epsilon)}} \right] \\
    &\leq \mathbb{E}\left[ (1-\epsilon)^{\frac{\sum_t \tilde{Y}_t}{\gamma \opt{}}} \right] / (1-\epsilon)^{\frac{1-\epsilon}{\gamma (1+\epsilon)}} \\
    &= \mathbb{E}\left[ \prod_t (1-\epsilon)^{\frac{\tilde{Y}_t}{\gamma \opt{}}} \right] / (1-\epsilon)^{\frac{1-\epsilon}{\gamma (1+\epsilon)}} \\
    &\leq \mathbb{E}\left[ \prod_t \left( 1-\epsilon \frac{\tilde{Y}_t}{\gamma \opt{}} \right) \right] / (1-\epsilon)^{\frac{1-\epsilon}{\gamma(1+\epsilon)}} \\
    &\leq \mathbb{E}\left[ \prod_t \left( 1 - \frac{\epsilon}{(1+\epsilon)\gamma m}\right) / (1-\epsilon)^{\frac{1-\epsilon}{\gamma (1+\epsilon)}} \right] \\
    &\leq \left( \frac{e^{-\epsilon}}{(1-\epsilon)^{1-\epsilon}}\right)^{1/\gamma(1+\epsilon)} \\
    &\leq e^{\frac{-e^2}{2\gamma(1+\epsilon)}} \\
    &\leq \frac{\epsilon}{n}
\end{align*} \todo{Explain how each inequality is achieved}
thus summing over all $n$ agents will give us a failure probability of $\geq 1-n \cdot \frac{\epsilon}{n} = 1-\epsilon$. This proves the main result:

\begin{theorem} \label{thm.known_comp}
    For any $\epsilon > 0$, the conservative algorithm $\tilde{P}$ achieves an objective value of $\opt{}(1-2\epsilon)$ for the online maxmin allocation problem with probability at least $1-\epsilon$, provided $\gamma = O\left( \frac{\epsilon^2}{\log (n/\epsilon)} \right)$
\end{theorem}

\subsubsection{Known \opt{}} We once again look to bound the error probability of our algorithm, and in this case produce a potential function for allocating impressions. Here we assume only knowledge of \opt{}. Let $A^s \tilde{P}^{m-s}$ be a hybrid algorithm which runs $A$ for the first $s$ iterations and algorithm $\tilde{P}$ from Section \ref{sec.known_dis} for the remaining $m-s$. We once again say the algorithm fails if $\sum_t Y_t \leq \opt{}(1-2\epsilon)$ for any $i \in D$. For better readability, let $S_s(Y_i) = \sum_t Y_i^A$ denote the profit in the first $s$ time steps using algorithm $A$. We can once again use a Chernoff bound to get the following inequality (see derivation in Section \ref{sec.known_dis}).
$$\mathbb{P}\left[ \sum_t Y_t \leq \frac{\opt{}}{1+\epsilon}(1-\epsilon)\right] \leq \mathbb{E}\left[ \prod_t (1-\epsilon)^{\frac{Y_t}{\gamma \opt{}}} \right] / (1-\epsilon)^{\frac{1-\epsilon}{\gamma (1+\epsilon)}}$$ which we can expand according to the first $s$ and final $m-s$ steps to produce
$$\frac{\mathbb{E}\left[(1-\epsilon)^{\frac{S_s(Y_i)}{\gamma \opt{}}} \prod_{t=s+1}^m (1-\epsilon)^{\frac{\tilde{Y}_{i,t}}{\gamma \opt{}}}\right]}{(1-\epsilon)^{\frac{1-\epsilon}{\gamma (1+\epsilon)}}}$$ now summing over $i$ we want to bound this by $\epsilon$:
$$\sum_i \frac{\mathbb{E}\left[(1-\epsilon)^{\frac{S_s(Y_i)}{\gamma \opt{}}} \prod_{t=s+1}^m (1-\epsilon)^{\frac{\tilde{Y}_{i,t}}{\gamma \opt{}}}\right]}{(1-\epsilon)^{\frac{1-\epsilon}{\gamma (1+\epsilon)}}} \leq \epsilon$$ and now we utilize the fact that $(1+\epsilon)^x \leq 1+\epsilon x$ for $0 \leq x \leq 1$ to upper bound the above by $$\sum_i \frac{\mathbb{E}\left[(1-\epsilon)^{\frac{S_s(Y_i)}{\gamma \opt{}}} \prod_{t=s+1}^m (1-\epsilon \frac{\tilde{Y}_{i,t}}{\gamma \opt{}})\right]}{(1-\epsilon)^{\frac{1-\epsilon}{\gamma (1+\epsilon)}}}$$ Since for all $t$, the variables $Y_{i,t}$ and $\tilde{Y}_{i,t}$ are independent and $\mathbb{E}[\tilde{Y}_{i,t}] \geq \frac{\opt{}}{(1+\epsilon)m}$ we can rewrite the summation as
\begin{align*}
    \sum_i \frac{\mathbb{E}\left[(1-\epsilon)^{\frac{S_s(Y_i)}{\gamma \opt{}}} (1-\frac{\epsilon}{(1+\epsilon)\gamma m})^{m-s}\right]}{(1-\epsilon)^{\frac{1-\epsilon}{\gamma (1+\epsilon)}}} \tag{B1} \label{eq.exp_ub}
\end{align*}
Denote the quantity in \ref{eq.exp_ub} $\mathcal{F}[A^s\tilde{P}^{m-s}]$ (an upperbound on the failure probability for the algorithm $A^s\tilde{P}^{m-s}$. We demonstrated in Theorem \ref{thm.known_comp} that $\mathcal{F}[\tilde{P}^m \leq \epsilon$ and we now want to derive an algorithm $A$ that has the same error bound.

Assuming that for all $s < p$, we have that $\mathcal{F}[A^{s+1}\tilde{P}^{m-s-1}] \leq \mathcal{F}[A^s\tilde{P}^{m-s}]$ and we seek to define $A$ for the $p+1$ step such that $\mathcal{F}[A^{p+1}\tilde{P}^{m-p-1}] \leq \mathcal{F}[A^p\tilde{P}^{m-p}]$:
\begin{align*}
    \mathcal{F}[A^{p+1}\tilde{P}^{m-p-1}] &= \sum_i \frac{\mathbb{E}\left[ (1-\epsilon)^{\frac{S_{p+1}(Y_i^A)}{\gamma \opt{}}} (1-\frac{\epsilon}{(1+\epsilon)\gamma m})^{m-p-1} \right]}{(1-\epsilon)^{\frac{1-\epsilon}{\gamma (1+\epsilon)}}} \\
    &\leq \sum_i \frac{\mathbb{E}\left[ (1-\epsilon)^{\frac{S_p(Y_i^A)}{\gamma \opt{}}}\left( 1 - \epsilon \frac{Y_{i,p+1}^A}{\gamma \opt{}} \right) (1-\frac{\epsilon}{(1+\epsilon)\gamma m})^{m-p-1} \right]}{(1-\epsilon)^{\frac{1-\epsilon}{\gamma (1+\epsilon)}}}
\end{align*}
We now define the following potential function:
\begin{align*}
    \phi_{i,s} = \frac{1}{\opt{}} \left[ \frac{(1-\epsilon)^{\frac{S_s(Y_i^A)}{\gamma \opt{}}} (1-\frac{\epsilon}{(1+\epsilon)\gamma m})^{m-s-1}}{(1-\epsilon)^{\frac{1-\epsilon}{\gamma(1+\epsilon)}}} \right]
\end{align*}
and define the $p+1$ step of our algorithm $A$ as picking the allocation that maximizes
$$\sum_i v_{i,p} \phi_{i,p}$$ We present this formally in Algorithm 1.

Now by definition of the above algorithm, for any two algorithms where the first $p$ steps are identical, and the last $m-p-1$ steps following $\tilde{P}$, algorithm A's $p+1$ step must minimize the sum over expectations. This gives us:
\begin{align*}
    \mathcal{F}[A^{p+1} \tilde{P}^{m-p-1}] &\leq \sum_i \frac{\mathbb{E}\left[ (1-\epsilon)^{\frac{S_p(Y_i^A)}{\gamma \opt{}}}\left( 1 - \epsilon \frac{\tilde{Y}_{i,p+1}^A}{\gamma \opt{}} \right) (1-\frac{\epsilon}{(1+\epsilon)\gamma m})^{m-p-1} \right]}{(1-\epsilon)^{\frac{1-\epsilon}{\gamma (1+\epsilon)}}} \\
    &\leq \sum_i \frac{\mathbb{E}\left[ (1-\epsilon)^{\frac{S_p(Y_i^A)}{\gamma \opt{}}}\left( 1 - \frac{\epsilon}{(1+\epsilon) \gamma \opt{}} \right) (1-\frac{\epsilon}{(1+\epsilon)\gamma m})^{m-p-1} \right]}{(1-\epsilon)^{\frac{1-\epsilon}{\gamma (1+\epsilon)}}} \\
    &= \mathcal{F}[A^p \tilde{P}^{m-p}]
\end{align*}
This completest the proof of the following:
\begin{theorem}
    For any $\epsilon > 0$, Algorithm 1 achieves an objective value of \opt{}$(1-2\epsilon)$ for the online allocation problem with probability at least $1-\epsilon$, assuming $\gamma = O\left(\frac{\epsilon^2}{\log(n/\epsilon)}\right)$
\end{theorem}

\begin{algorithm}[tb]
\caption{Restricted Assignment with Unknown Distribution}
\label{alg:algorithm}
\begin{algorithmic}[1]
\STATE Initialize $\phi_{i,0} = \frac{1}{\opt{}}\left[ \frac{(1-\frac{\epsilon}{(1+\epsilon)\gamma m})^{m-1}}{(1-\epsilon)^{\frac{1-\epsilon}{\gamma(1+\epsilon)}}} \right]$
\FOR{$t = 1$ to $m$}
    \STATE Allocate request according to $$\max_i \sum_i w_{i,t-1} \phi_{i,t-1}$$
\STATE $Y_{i,t}^A = v_{i^* j}$
\STATE Update $\phi_{i,t} = \phi_{i,t-1} \cdot \left[ \frac{(1-\epsilon)^{\frac{Y_{i,t}^A}{\gamma \opt{}}}}{1 - \frac{\epsilon}{(1+\epsilon)\gamma m}} \right]$
\ENDFOR
\end{algorithmic}
\end{algorithm}

\subsubsection{No known values}

\subsection{Agrawal/Devanur Method} It seems we could implement this multiplicate weights / experts algorithm with a proper smoothing of the maximum function. As such, it would make sense to use $$\textsc{LogSumExp}(\bold x) = \log(\exp(x_1) + \exp(x_2) + ... + \exp(x_n))$$ since it is convex (and moreso strongly convex if we modify slightly to include an $n+1$ coordinate that is set to 0). This function is very standard smoothing. To adapt the algorithm to capture the \emph{minimum}, we use
$$\min\{\bold x\} - \leq \frac{-1}{\epsilon}\textsc{LSE}(-\epsilon \bold{x}) \leq \min\{\bold x\}$$ which is our objective function to maximize over (or maximize the average value of in the case of OCO method).
\end{document}

==> TrashFiles/prelim.tex <==
In this section, we introduce the notation that we will use in the rest of the paper. Let $\bA^1, ..., \bA^m$ denote the input sequence of items arriving in random order where each $\bA^j$ is an $n \times n$ diagonal matrix where the diagonal entries corresponds to that agents value for the item (which are assumed to be in $[0,1]$). We can thus let $\bx^1, ... , \bx^m \in [0,1]^n$ denote the fractional allocation of the algorithm, giving the value vector $\bA^j \bx^j$ for the $j$-th item's allocation.
%
We further let the corresponding allocations of a fixed (offline) optimal solution be denoted as $\xopt^1, ..., \xopt^m \in [0,1]^n$ and let $\opt{}$ denote the max-min objective value of the optimal solution. Lastly, we define $\bv^t = \sum_{\tau=1}^t \bA^\tau \bx^\tau = (v_1^t, ..., v_n^t)$ be the vector of agent's allocation values up to time $t$. Our problem thus amounts to maximizing the component-wise minimum of $\bv^m$.
%$i$-th column of such a matrix which represents the value of item $j$ for agent $i$. Furthermore, this vector can only have a nonzero value in the $i$-th position: $\bA_{i}^j = (0,...,0,v_{ij},0,...,0)^T$. 
We again note that in the random-order input model, an adversary selects the set $\{\bA^1, ..., \bA^m\}$ but the sequence {\em order} is random.

==> TrashFiles/random-scalar.tex <==
In this section, we present the approximately greedy algorithm, Algorithm \ref{alg:smooth_greedy}, and analyze its competitive ratio in the random order model. Building on the work of Molinaro for online scheduling~\cite{Molinaro_2017}, we use a greedy algorithm for a smoothed version of our objective function and a restart procedure during the online allocation process to reduce the impact of correlations that arise in this input model. %The analysis that follows can be interpreted as the dual equivalent of Molinaro~\cite{Molinaro_2017} for our concave objective. %Though, in general, algorithms for maximization and minimization do not align, we show that for our online problem the results are essentially equivalent.

A natural strategy for our problem is to allocate the arriving item to the least satisfied agent. However, one can show this strategy has too high an additive regret \cite{Gupta_2014, Molinaro_2017} as the change in our solution value can vary quickly from one iteration to the next. Instead, we use a \emph{smoothed} version of the greedy algorithm. The algorithm is designed as follows: we first define $\phi_\ve$ to be a re-scaled variant of the \textsc{LogSumExp} function that serves as a smoothed minimum. For the first half of the input stream, we select an allocation for each arriving item that maximizes the increase in our smoothed objective function. This stage can be thought of as approximately greedy with respect to the \emph{gradient} of $\phi_\ve$. After $\frac{m}{2}$ items have been allocated, we ``restart'' the allocation by maximizing the increase in our objective with respect to the $t > \frac{m}{2}$ allocations only. This restart procedure is essential for reducing the correlations that arise in sampling without replacement in the random order model since at each iteration of the allocation procedure, our decision depends on at most $\frac{m}{2}-1$ items. The pseudocode of this procedure is presented in Algorithm \ref{alg:smooth_greedy}.

\begin{algorithm}[b]
	\SetAlgoNoLine
	\KwIn{$0 < \ve < 1$, input stream $\mathcal{M}$ of $m$ items}
	\KwOut{$(1-\ve)$-competitive \textsc{MaxMin} allocation}
	Define $\phi_\ve(u) = \frac{-1}{\ve} \ln \left(\sum_i e^{-\ve u_i}\right)$\;
	\For{$t=1$ to $m/2$}
	{
	    Select $\bx^t \in \Delta^n$ to maximize $\phi_\ve \left(\sum_{\tau = 1}^t \bV^{\tau} \right)$\;
	}
	\For{$t=m/2 + 1$ to $m$}
	{
	    Select $\bx^t \in \Delta^n$ to maximize $\phi_\ve \left(\sum_{\tau = \frac{m}{2} + 1}^t \bV^{\tau} \right)$\;
	}
	\caption{\textsc{Smooth Greedy With Restart}}
	\label{alg:smooth_greedy}
\end{algorithm}

\subsection{Algorithm Analysis}

In the analysis of the competitive ratio of Algorithm \ref{alg:smooth_greedy}, we will leverage several key facts about the smoothed minimum function $\phi_\ve$. Allocating with respect to this function produces an almost greedy process on the function's gradient, allowing us to follow the analysis of \cite{AgraDev_2014,devanur2009adwords,Molinaro_2017} to get the desired guarantees for the random-order model. We now state our main result in Theorem \ref{thm:ROM}.

\begin{theorem} \label{thm:ROM}
    For any $\ve > 0$, Algorithm \ref{alg:smooth_greedy} guarantees in the random-order input model that the expected value of the allocation assigned to any agent is at least
    $$(1 - \ve)\cdot  \opt{} - O \left( \frac{\log n}{\ve} \right).$$
\end{theorem}
Note that this theorem immediately implies the following corollary since the additive regret term can be absorbed in the multiplicative error for sufficiently large $\opt$:
\begin{corollary}
    For any $\ve > 0$, Algorithm \ref{alg:smooth_greedy} has a competitive ratio of $(1-\e)$ for $\opt \ge \Omega\left(\frac{\log n}{\ve^2}\right)$.
\end{corollary}

In order to prove this theorem, we first show some properties of the smoothed minimum function $\phi_\ve$ utilized by Algorithm \ref{alg:smooth_greedy}. We will then prove some technical lemmas that will help establish the theorem.

Lemma \ref{lem:props} effectively defines the additive error with respect to our true objective, the agent-wise minimum, and stability of the smooth function following each allocation decision. As was shown in prior work, allocating with respect to the order statistics or even the $L_p^p$ norm produces either too high of a regret factor, or instability in the derivative value under small perturbations to the input value. As such, the smoothing and the following properties are critical to maintaining our regret and competitive ratio bounds.
\begin{lemma} \label{lem:props}
    For all $u \in \mathbb{R}^n$, $v \in [0,1]^n$, and $\ve > 0$, the function $\phi_\ve(x) = \frac{-1}{\ve}\ln \left( \sum_{i=1}^n e^{-\ve x_i} \right)$ satisfies the following:
    \begin{itemize}
        \item[(a)] $\min_i \{u_i\} - \frac{\ln n}{\ve} \leq \phi_\ve(u) < \min_i \{u_i\}$
        \item[(b)] $\nabla \phi_\ve (u + v) \in e^{\pm \ve} \cdot \nabla \phi_\ve (u)$
    \end{itemize}
\end{lemma}
The proof of these properties are deferred to Appendix \ref{sec:omitted} due to space constraints.

Now utilizing these two properties we can prove the following important bound on the inner product of the smoothed minimum's gradient. This will be used throughout our analysis to bound the incremental change in the objective \textsc{MaxMin} value after each allocation decision, and the summation of these changes can be seen as the accumulated ``reward'' at any given stage of the input stream. The proof is by direct integration of stability property $(b)$ and is thus deffered to Appendix \ref{sec:omitted}.

\begin{lemma} \label{lem:grad_bound}
    For $u \in \mathbb{R}^n$ and $v,v' \in [0,1]^n$, if $\phi_\ve(u + v) \geq \phi_\ve (u + v')$ then $\langle \nabla \phi_\ve(u), v \rangle \geq e^{-2\ve} \langle \nabla \phi_\ve(u), v' \rangle$.
\end{lemma}

We now follow in the intuition of Agrawal and Devanur \cite{AgraDev_2014} to prove Theorem \ref{thm:ROM} by bounding the incremental increase in our ``reward'' both before and after the restart at $t = \frac{m}{2}$. By implementing this restart in the allocation procedure, we segment the stream into two portions that have identical probabilistic guarantees and reduce the correlation between input elements to allow for an optimal competitive ratio and low additive regret.

\begin{proof}[Proof of Theorem \ref{thm:ROM}]
    We note again that in the approximately greedy procedure of Algorithm \ref{alg:smooth_greedy}, we are essentially seleting items greedily according to the \emph{gradient} of $\phi_\ve$ to maximize the incremental changes. Due to the restart at $m/2$, we define 
    \begin{gather*}
        \nabla^t = \nabla \phi_\ve\left(\sum_{\tau=1}^{t-1}\bV^{\tau}\right) \text{ for } t \leq \frac{m}{2} \text{ and } \nabla^t = \nabla \phi_\ve\left(\sum_{\tau=m/2 + 1}^{t-1}\bV^{\tau}\right) \text{ for } t > \frac{m}{2}
    \end{gather*}
    We now proceed by deriving a bound on $\min_i \{\sum_{\tau=1}^m\bV^{\tau}_{i}\}$ in terms of our smoothed-approximation function $\phi_\ve$, thus bounding the accumulated error by the algorithm when estimating our true objective. By the concavity of $\phi_\ve$ and Lemma \ref{lem:props}, we have that
    \begin{align*}
        \phi_\ve\left(\sum_{\tau=1}^t\bV^{\tau}\right) - \phi_\ve\left(\sum_{\tau=1}^{t-1}\bV^{\tau}\right) &\geq \left\langle \nabla \phi_\ve\left(\sum_{\tau=1}^t\bV^{\tau}\right), \bV^t \right\rangle \tag{Concavity} \\
        &\geq e^{-\ve} \left\langle \nabla \phi_\ve\left(\sum_{\tau=1}^{t-1}\bV^{\tau}\right), \bV^t \right\rangle \tag{Lemma \ref{lem:props}} \\
        &= e^{-\ve} \langle \nabla^{t}, \bV^t \rangle.
    \end{align*}
    Without loss of generality we proceed by considering the first half of the input sequence ($t \leq \frac{m}{2}$). By summing this inequality over the input stream prior to the restart (from $t=1$ to $\frac{m}{2}$), we have
    \begin{align*}
        \phi_\ve\left(\sum_{\tau=1}^{m/2}\bV^{\tau}\right) - \phi_\ve\left(\bV^0\right) \geq e^{-\ve} \sum_{t=1}^{m/2} \langle \nabla^{t}, \bV^t \rangle.
    \end{align*}
    Furthermore, we have that $\phi_\ve(0) = \frac{-\ln n}{\ve}$ and thus the inequality becomes
    \begin{align}
        \phi_\ve\left(\sum_{\tau=1}^{m/2}\bV^{\tau}\right) + \frac{\ln n}{\ve} \geq  e^{-\ve} \sum_{t=1}^{m/2} \langle \nabla^{t}, \bV^t\rangle \label{lem:olo_ineq}
    \end{align}
    Now, taking into account the allocation before and after the restart at $\frac{m}{2}$ and invoking Eq.~\eqref{lem:olo_ineq} for each half of the input stream with the concavity of $\phi_\ve$, we obtain
    \begin{align*}
        \sum_{t=1}^m \langle \nabla^{t}, \bV^t \rangle &\leq e^\ve \left( \phi_\ve\left(\sum_{\tau=1}^{m/2}\bV^{\tau}\right) + \phi_\ve\left(\sum_{\tau=m/2 + 1}^{m}\bV^{\tau}\right) + \frac{2 \ln n}{\ve}\right) \tag{Ineq. \ref{lem:olo_ineq}}\\
        &\leq e^\ve \left( \phi_\ve\left(\sum_{\tau=1}^{m}\bV^{\tau}\right) + \frac{2 \ln n}{\ve}\right) \tag{Concavity} \\
        &\leq e^\ve \left( \min_i \{\sum_{\tau=1}^{m}\bV_i^{\tau}\} + \frac{2 \ln n}{\ve}\right) \tag{Lemma \ref{lem:props}}
    \end{align*}
    where the last inequality is a direct result of Lemma \ref{lem:props}. Lastly, by rearranging terms we can bound the element-wise minimum as
    \begin{align}
        \min_i \{\sum_{\tau=1}^{m}\bV_i^{\tau}\} \geq e^{-\ve} \left( \sum_{t=1}^m \langle \nabla^{t}, \bV^t\rangle \right) - \frac{2 \ln n}{\ve}. \label{ineq:min_bound}
    \end{align}
    Thus, the output of our algorithm will approximate the \emph{actual} objective function within a multiplicative factor of $e^{-\ve} \approx 1-\ve$ and an additive regret on the order of $\ln n / \ve$. 
    
    We now proceed to bound the gap between our algorithmic solution to that of the optimal \emph{offline} solution which, combined with the above error, will give the final result.
    %
    As such, the final step of our analysis will be to take the expectation of this inequality to get the final bounds in Theorem \ref{thm:ROM}. Due to the restart and random order input model, the expected increase in maximal value over the first and second half is equivalent, $$\Ex\left[ \sum_{t=1}^{m/2} \langle \nabla^{t}, \bV^t\rangle\right] = \Ex\left[ \sum_{t=m/2+1}^{m} \langle \nabla^{t}, \bV^t\rangle\right]$$ so without loss of generality we need only bound the first half's value and apply this bound to both portions. The benefit of this restart will yield a tolerable error as compared to the optimal offline solution in each half of the allocation procedure, rather than a continuously accumulating divergence between the two solutions. 
    
    Now, by the nature of greedy selection to maximize our objective function, we must have that in each iteration our algorithm's selection has value at least as good as that of the optimal offline solution $\phi_\ve\left(\bV^t\right) \geq \phi_\ve(\bVo^t)$ for each $t$. Combining this with Lemma \ref{lem:grad_bound}, we must have 
    $$\langle \nabla^t, \bV^t \rangle \geq e^{-2\ve} \langle \nabla^t, \bVo^t \rangle$$
    Furthermore, since $\nabla \phi_\ve \in \ell_1$ \cite{gao2017properties} and $\nabla^t$ is independent of $\bV^t$, we prove the following purely probabilistic result that will be used to bound the above summations to derive the final result.
    \alert{The lemma below is a slight extension of a lemma from \cite{Gupta_2014} so maybe can defer proof to appendix for space}
    \begin{lemma} \label{lem:hoeff}
    Consider a set of vectors $\{y^1, ..., y^m\} \in [0,1]^n$ and let $\bY^1, ..., \bY^k$ be sampled without replacement from this set. Let $\bZ \in \ell_1^+$ be a random unit-vector that depends only on $\bY^1, ..., \bY^{k-1}$. Then for all $\ve > 0$,
    $$\Ex\langle \bY^k, \bZ \rangle \geq e^{-\ve} \min_i \{\Ex\bY^k_i\} - \frac{\ln n}{\ve \left(m - k + 1 \right)}.$$
    \end{lemma}
    %
    \eat{
    Intuitively, this lemma demonstrates the vitality of the reduction in correlation between items arriving in the online stream as a result of the restart in our algorithm. If, instead, $\bZ$ were highly dependent on $\bY^k$, in the worst case $\Ex \langle \bY^k, \bZ \rangle = \Ex \left[ \min_i \bY^k_i \right]$ which can be substantially greater than $\min_i \{\Ex \bY_i^k\}$.
    }
    %
    \begin{proof}
    Let $\mu = \frac{1}{m} \sum_t y^t$ be the average of the set of vectors and to simplify notation we additionally break apart the expectation and let $\Ex\langle \bY^k, \bZ \rangle = \Ex \left[ \Ex \left[ \langle \bY^k, \bZ \rangle | \bY^1, ..., \bY^{k-1} \right] \right]$. Note that since $\bZ$ is a unit-vector in $\ell_1^+$, an innerproduct of this vector with $\bY^k$ is simply a weighted sum of the latter's elements. Thus, we have
    \begin{align} \label{ineq.inner_prod}
        \Ex\left[ \langle \bY^k, Z \rangle | \bY^1, ..., \bY^{k-1} \right] %&=  \langle \Ex\left[\bY^k | \bY^1, ..., \bY^{k-1} \right], Z \rangle \\
        \geq \min_i \{ \Ex \left[ \bY^k | \bY^1, ..., \bY^{k-1}\right] \}.
    \end{align}
    Additionally, by nature of the sampling set and the procedure of sampling without replacement, we have the conditional expectation
    $$\Ex\left[ \bY^k | \bY^1, ..., \bY^{k-1} \right] = \frac{m\mu - (\bY^1 + ... + \bY^{k-1})}{m - (k - 1)}$$ and further note that $m\mu - (\bY^1 + ... + \bY^{k-1})$ has the \emph{same} distribution as $\bY^1 + ... + \bY^{m-(k-1)}$. This concretely gives us the simplifying equivalences
    $$\Ex\left[ \bY^k | \bY^1, ..., \bY^{k-1} \right] = \frac{m\mu - (\bY^1 + ... + \bY^{k-1})}{m-(k-1)} = \frac{\sum_{t=1}^{m-(k-1)} \bY^t}{m-(k-1)}.$$
    % and thus $\Ex\left[ \bY^k | \bY^1, ..., \bY^{k-1} \right]$ has the same distribution as $\frac{\bY^1 + ... \bY^{m-(k-1)}}{m - (k-1)}$. 
    %
    % Now taking expectations, we have
    %$$\Ex \left[ \min_i \{ \Ex\left[ \bY^k_i | \bY^1, ..., \bY^{k-1} \right] \} \right] = \frac{1}{m - (k - 1)}\Ex\left[ \min_i \{ \Ex\left[ \bY^1_i + ... + \bY^{m - (k - 1)}_i \right] \} \right]$$
    % Now noting that $\nabla^k \in \ell_1^+$ in Algorithm \ref{alg:smooth_greedy}, we can use Inequality (\ref{ineq:min_bound}) here and taking expectations we have
    % To bound this value, we invoke Inequality (\ref{ineq:min_bound}) and taking expectations we have
    % $$\sum_{t \leq k} \Ex \langle \bY^t, \bZ^t \rangle \leq e^\ve \left( \Ex \left[ \min_i \{ \sum_{t \leq k} \bY^t \}  \right] + \frac{\log n}{\ve}\right)$$
    We now return to the inequality bound of (\ref{ineq.inner_prod}) and, using the above equivalences, obtain 
    \begin{align*}
        \Ex \left[ \min_i \left\{ \sum_{t=1}^{m-(k-1)} \bY_i^t \right\} \right] &\geq \Ex \left[ \phi_\ve \left(\Sigma_{t=1}^{m-(k-1)} \bY^t \right) \right] \tag{Lemma \ref{lem:props}}\\
        &= \Ex \left[\frac{-1}{\ve} \ln \left( \sum_i \exp{\left(-\ve \Sigma_{t=1}^{m-(k-1)} \bY_i^t\right)} \right) \right]\\
        &\geq \frac{-1}{\ve} \ln \left( \sum_i \exp{\left(-\ve \Ex \left[ \Sigma_{t=1}^{m-(k-1)} \bY_i^t \right]\right)} \right) \tag{Jensen's Ineq.} \\
        &\geq e^{-\ve} \min_i \left\{ \Ex [\Sigma_{t=1}^{m-(k-1)} \bY_i^t] \right\} - \frac{\ln n}{\ve} \tag{Lemma \ref{lem:props}} \\
        &\geq e^{-\ve} \min_i \left\{ (m-(k-1)) \Ex \bY_i^t \right\} - \frac{\ln n}{\ve}
    \end{align*}
    %$$\Ex \left[ \min_i \{ \sum_{t=1}^{m-(k-1)} \bY^t \} \right] \geq e^{-\ve} \min_i \{ (m-(k-1)) \Ex \bY^t \} - \frac{\log n}{\ve}$$
    % \todo{cite this Chernoff result}
    
    \begin{comment}
    and since $\bZ^t$ is independent of $\bY^t$, we have $\Ex \langle \bY^t, \bZ^t \rangle = \langle \Ex \bY^t, \Ex\bZ^t \rangle.$ Thus, we can lower bound the left-hand side of the above inequality in the following manner:
    \begin{align*}
        \sum_{t \leq k} \Ex \langle \bY^t, \bZ^t \rangle &= \sum_{t \leq k} \langle \Ex \bY^t, \Ex \bZ^t  \rangle  \\
        &= \sum_{t \leq k} \langle \frac{\mu}{m} , \Ex \bZ^t \rangle \\
        &= \langle \mu, \frac{1}{m} \sum_{t \leq k} \bZ^t \rangle \\
        &\geq \min_i \{\mu_i\} \\
        &= \min_i \{\sum_{t \leq k} \Ex \bY^t\}
    \end{align*}
    where the inequality \todo{. . .}. Therefore, we have that $$\Ex \left[ \min_i \{ \sum_{t \leq m-(k-1)} \bY^t \}  \right] \geq e^{-\ve} \min_i \{\sum_{t \leq k} \Ex \bY^t\} - \frac{\ln n}{\ve}$$
\end{comment}
    
    \noindent %where the first and third inequalities come from Lemma \ref{lem:props}, and the second from repeated application of Jensen's inequality. 
    Finally combining the above results, we obtain
    \begin{align*}
        \frac{1}{m-(k-1)} \left(e^{-\ve} \min_i \{ (m-(k-1)) \Ex \bY^t \} - \frac{\ln n}{\ve} \right) &\leq \Ex \left[ \min_i \{\Ex \left[\bY^k_i | \bY^1, ..., \bY^{k-1} \right] \} \right] \\
        &\leq \Ex \langle \bY^t, \bZ \rangle
    \end{align*}
    Thus, after rearranging terms, this completes the lemma.
    \end{proof}
    
    \noindent Using this lower bounding result, we can now bound the sum of rewards as
    \begin{align} \label{ineq.opt_lb}
        \Ex\left[ \langle \nabla^t, \bVo^t \rangle \right] \geq e^{-\ve} \min_i \{\Ex\left[ \bVo^t_i \right]\} - \frac{\ln n}{\ve(m - t + 1)}.
    \end{align}
    Adding this result over all $t \leq \frac{m}{2}$ in combination with $\min_i \{\Ex\left[ \bVo^t \right]_i\} = \frac{\opt{}}{m}$ we conclude that 
    \begin{align*}
        e^{2\ve} \cdot \Ex \sum_{t \leq \frac{m}{2}} \langle \nabla^t, \bV^t \rangle &\geq \Ex \sum_{t \leq \frac{m}{2}} \langle \nabla^t, \bVo^t \rangle \tag{Lemma \ref{lem:props}} \\
        &\geq e^{-\ve} \sum_{t \leq \frac{m}{2}} \min_i \{\Ex\left[ \bVo^t_i \right]\} - \sum_{t \leq \frac{m}{2}} \frac{\ln n}{\ve(m - t + 1)}  \tag{Ineq. \ref{ineq.opt_lb}}\\
        &= e^{-\ve} \left( \frac{\opt{}}{2}\right) - \frac{\ln n}{\ve}
    \end{align*}
    Due to the restart at $t = \frac{m}{2}$, we can extend the sum to $t = m$ by simply multiplying the above RHS by two. Finally, invoking inequality (\ref{ineq:min_bound}), we see that
    $$\Ex\left[ \min_i \sum_{\tau=1}^m\bV^{\tau} \right] \geq e^{-4\ve} \opt{} - O \left(\frac{\log n}{\ve}\right) \geq \left(1-O(\ve)\right) \opt{} - O\left(\frac{\log n }{\ve}\right).$$
    by the Taylor approximation $e^{-x} \geq 1-x$ and the assumption on the size of \opt{}.\\ % \todo{randomized rounding of solution}
\end{proof}

==> TrashFiles/random.tex <==
In this section, we present the approximately greedy algorithm, Algorithm \ref{alg:smooth_greedy}, and analyze its competitive ratio in the random order model. Building on the work of Molinaro for online scheduling~\cite{Molinaro_2017}, we use a greedy algorithm for a smoothed version of our objective function and a restart procedure during the online allocation process to reduce the impact of correlations that arise in this input model. %The analysis that follows can be interpreted as the dual equivalent of Molinaro~\cite{Molinaro_2017} for our concave objective. %Though, in general, algorithms for maximization and minimization do not align, we show that for our online problem the results are essentially equivalent.

A natural strategy for our problem is to allocate the arriving item to the least satisfied agent. However, one can show this strategy has too high an additive regret \cite{Gupta_2014, Molinaro_2017} as the change in our solution value can vary quickly from one iteration to the next. Instead, we use a \emph{smoothed} version of the greedy algorithm. The algorithm is designed as follows: we first define $\phi_\ve$ to be a re-scaled variant of the \textsc{LogSumExp} function that serves as a smoothed minimum. For the first half of the input stream, we select an allocation for each arriving item that maximizes the increase in our smoothed objective function. This stage can be thought of as approximately greedy with respect to the \emph{gradient} of $\phi_\ve$. After $\frac{m}{2}$ items have been allocated, we ``restart'' the allocation by maximizing the increase in our objective with respect to the $t > \frac{m}{2}$ allocations only. This restart procedure is essential for reducing the correlations that arise in sampling without replacement in the random order model since at each iteration of the allocation procedure, our decision depends on at most $\frac{m}{2}-1$ items. The pseudocode of this procedure is presented in Algorithm \ref{alg:smooth_greedy}.

\eat{
\subsection{Input Model}

Before presenting the algorithm, we define some notation specific to the input model. Let $\bA^1, ..., \bA^m$ denote the input sequence of items arriving in random order where each $\bA^j$ is an $n \times n$ matrix defining the value vectors of the impression to each agent. More concretely, let $\bA_{i}^j$ denote the $i$-th column of such a matrix which represents the value of impression $j$ to agent $i$. Furthermore, this vector can only have a nonzero value in the $i$-th position: $\bA_{i}^j = (0,...,0,v_{ij},0,...,0)^T$. We again note that in the random-order input model, an adversary selects each of the $\bA^j$ but is not permitted to select the \emph{order} that they arrive in. This allows for substantially improved guarantees over the adversarial input model. We additionally let $\bx^1, ... , \bx^m \in [0,1]^n$ denote the allocation decisions output by the algorithm which are compared against the allocations made by the optimal offline solution, $\xopt^1, ..., \xopt^m \in [0,1]^n$. Lastly, we let $\bv^t = \sum_{\tau=1}^t \bA^\tau \bx^\tau = (v_1^t, ..., v_n^t)$ be the vector of agent's allocation values up to time $t$. Our problem thus amounts to maximizing the component-wise minimum of $\bv^m$.
}


\begin{algorithm}[b]
	\SetAlgoNoLine
	\KwIn{$0 < \ve < 1$, input stream $\mathcal{M}$ of $m$ items}
	\KwOut{$(1-\ve)$-competitive \textsc{MaxMin} allocation}
	Define $\phi_\ve(u) = \frac{-1}{\ve} \ln \left(\sum_i e^{-\ve u_i}\right)$\;
	\For{$t=1$ to $m/2$}
	{
	    Select $\bx^t \in \Delta^n$ to maximize $\phi_\ve \left(\sum_{\tau = 1}^t \bA^\tau x^\tau \right)$\;
	}
	\For{$t=m/2 + 1$ to $m$}
	{
	    Select $\bx^t \in \Delta^n$ to maximize $\phi_\ve \left(\sum_{\tau = \frac{m}{2} + 1}^t \bA^\tau x^\tau \right)$\;
	}
	\caption{\textsc{Smooth Greedy With Restart}}
	\label{alg:smooth_greedy}
\end{algorithm}

\subsection{Algorithm Analysis}

In the analysis of the competitive ratio of Algorithm \ref{alg:smooth_greedy}, we will leverage several key facts about the smoothed minimum function $\phi_\ve$. Allocating with respect to this function produces an almost greedy process on the function's gradient, allowing us to follow the analysis of \cite{AgraDev_2014,devanur2009adwords,Molinaro_2017} to get the desired guarantees for the random-order model. We now state our main result in Theorem \ref{thm:ROM}.

\begin{theorem} \label{thm:ROM}
    For any $\ve > 0$, Algorithm \ref{alg:smooth_greedy} guarantees in the random-order input model that the expected value of the allocation assigned to any agent is at least
    $$(1 - \ve)\cdot  \opt{} - O \left( \frac{\log n}{\ve} \right).$$
\end{theorem}
Note that this theorem immediately implies the following corollary since the additive regret term can be absorbed in the multiplicative error for sufficiently large $\opt$:
\begin{corollary}
    For any $\ve > 0$, Algorithm \ref{alg:smooth_greedy} has a competitive ratio of $(1-\e)$ for $\opt \ge \Omega\left(\frac{\log n}{\ve^2}\right)$.
\end{corollary}

In order to prove this theorem, we first show some properties of the smoothed minimum function $\phi_\ve$ utilized by Algorithm \ref{alg:smooth_greedy}. We will then prove some technical lemmas that will help establish the theorem.

Lemma \ref{lem:props} effectively defines the additive error with respect to our true objective, the agent-wise minimum, and stability of the smooth function following each allocation decision. As was shown in prior work, allocating with respect to the order statistics or even the $L_p^p$ norm produces either too high of a regret factor, or instability in the derivative value under small perturbations to the input value. As such, the smoothing and the following properties are critical to maintaining our regret and competitive ratio bounds.
\begin{lemma} \label{lem:props}
    For all $u \in \mathbb{R}^n$, $v \in [0,1]^n$, and $\ve > 0$, the function $\phi_\ve(x) = \frac{-1}{\ve}\ln \left( \sum_{i=1}^n e^{-\ve x_i} \right)$ satisfies the following:
    \begin{itemize}
        \item[(a)] $\min_i \{u_i\} - \frac{\ln n}{\ve} \leq \phi_\ve(u) < \min_i \{u_i\}$
        \item[(b)] $\nabla \phi_\ve (u + v) \in e^{\pm \ve} \cdot \nabla \phi_\ve (u)$
    \end{itemize}
\end{lemma}
The proof of these properties are deferred to Appendix \ref{sec:omitted} due to space constraints.

Now utilizing these two properties we can prove the following important bound on the inner product of the smoothed minimum's gradient. This will be used throughout our analysis to bound the incremental change in the objective \textsc{MaxMin} value after each allocation decision, and the summation of these changes can be seen as the accumulated ``reward'' at any given stage of the input stream. The proof is by direct integration of stability property $(b)$ and is thus deffered to Appendix \ref{sec:omitted}.

\begin{lemma} \label{lem:grad_bound}
    For $u \in \mathbb{R}^n$ and $v,v' \in [0,1]^n$, if $\phi_\ve(u + v) \geq \phi_\ve (u + v')$ then $\langle \nabla \phi_\ve(u), v \rangle \geq e^{-2\ve} \langle \nabla \phi_\ve(u), v' \rangle$.
\end{lemma}

We now follow in the intuition of Agrawal and Devanur \cite{AgraDev_2014} to prove Theorem \ref{thm:ROM} by bounding the incremental increase in our ``reward'' both before and after the restart at $t = \frac{m}{2}$. By implementing this restart in the allocation procedure, we segment the stream into two portions that have identical probabilistic guarantees and reduce the correlation between input elements to allow for an optimal competitive ratio and low additive regret.

\begin{proof}[Proof of Theorem \ref{thm:ROM}]
    We note again that in the approximately greedy procedure of Algorithm \ref{alg:smooth_greedy}, we are essentially seleting items greedily according to the \emph{gradient} of $\phi_\ve$ to maximize the incremental changes. Due to the restart at $m/2$, we define 
    \begin{gather*}
        \nabla^t = \nabla \phi_\ve(\bv^{t-1}) \text{ for } t \leq \frac{m}{2} \text{ and } \nabla^t = \nabla \phi_\ve(\bv^{t-1} - \bv^{m/2}) \text{ for } t > \frac{m}{2}
    \end{gather*}
    We now proceed by deriving a bound on $\min_i \{\bv^m_{i}\}$ in terms of our smoothed-approximation function $\phi_\ve$, thus bounding the accumulated error by the algorithm when estimating our true objective. By the concavity of $\phi_\ve$ and Lemma \ref{lem:props}, we have that
    \begin{align*}
        \phi_\ve(\bv^t) - \phi_\ve(\bv^{t-1}) &\geq \langle \nabla \phi_\ve(\bv^t), \bA^t \bx^t\rangle \\
        &\geq e^{-\ve} \langle \nabla \phi_\ve(\bv^{t-1}), \bA^t \bx^t\rangle \\
        &= e^{-\ve} \langle \nabla^{t}, \bA^t \bx^t\rangle.
    \end{align*}
    Without loss of generality we proceed by considering the first half of the input sequence ($t \leq \frac{m}{2}$). By summing this inequality over the input stream prior to the restart (from $t=1$ to $\frac{m}{2}$), we have
    \begin{align*}
        \phi_\ve(\bv^{m/2}) - \phi_\ve(\bv^0) \geq e^{-\ve} \sum_{t=1}^{m/2} \langle \nabla^{t}, \bA^t \bx^t\rangle.
    \end{align*}
    Furthermore, we have that $\phi_\ve(0) = \frac{-\ln n}{\ve}$ and thus the inequality becomes
    \begin{align}
        \phi_\ve(\bv^{m/2}) + \frac{\ln n}{\ve} \geq  e^{-\ve} \sum_{t=1}^{m/2} \langle \nabla^{t}, \bA^t \bx^t\rangle \label{lem:olo_ineq}
    \end{align}
    Now, taking into account the allocation before and after the restart at $\frac{m}{2}$ and invoking Eq.~\eqref{lem:olo_ineq} for each half of the input stream with the concavity of $\phi_\ve$, we obtain
    \begin{align*}
        \sum_{t=1}^m \langle \nabla^{t}, \bA^t \bx^t\rangle &\leq e^\ve \left( \phi_\ve(\bv^{m/2}) + \phi_\ve(\bv^{m} - \bv^{m/2}) + \frac{2 \ln n}{\ve}\right)\\
        &\leq e^\ve \left( \phi_\ve(\bv^{m}) + \frac{2 \ln n}{\ve}\right) \\
        &\leq e^\ve \left( \min_i \{\bv_i^m\} + \frac{2 \ln n}{\ve}\right)
    \end{align*}
    where the last inequality is a direct result of Lemma \ref{lem:props}. Lastly, by rearranging terms we can bound the element-wise minimum as
    \begin{align}
        \min_i \{\bv_i^m\} \geq e^{-\ve} \left( \sum_{t=1}^m \langle \nabla^{t}, \bA^t \bx^t\rangle \right) - \frac{2 \ln n}{\ve}. \label{ineq:min_bound}
    \end{align}
    Thus, the output of our algorithm will approximate the \emph{actual} objective function within a multiplicative factor of $e^{-\ve} \approx 1-\ve$ and an additive regret on the order of $\ln n / \ve$. 
    
    We now proceed to bound the gap between our algorithmic solution to that of the optimal \emph{offline} solution which, combined with the above error, will give the final result.
    %
    As such, the final step of our analysis will be to take the expectation of this inequality to get the final bounds in Theorem \ref{thm:ROM}. Due to the restart and random order input model, the expected increase in maximal value over the first and second half is equivalent, $$\Ex\left[ \sum_{t=1}^{m/2} \langle \nabla^{t}, \bA^t \bx^t\rangle\right] = \Ex\left[ \sum_{t=m/2+1}^{m} \langle \nabla^{t}, \bA^t \bx^t\rangle\right]$$ so without loss of generality we need only bound the first half's value and apply this bound to both portions. The benefit of this restart will yield a tolerable error as compared to the optimal offline solution in each half of the allocation procedure, rather than a continuously accumulating divergence between the two solutions. 
    
    Now, by the nature of greedy selection to maximize our objective function, we must have that in each iteration our algorithm's selection has value at least as good as that of the optimal offline solution $\phi_\ve(\bA^t\bx^t) \geq \phi_\ve(\bA^t\xopt^t)$ for each $t$. Combining this with Lemma \ref{lem:grad_bound}, we must have 
    $$\langle \nabla^t, \bA^t \bx^t \rangle \geq e^{-2\ve} \langle \nabla^t, \bA^t \xopt^t \rangle$$
    Furthermore, since $\nabla \phi_\ve \in \ell_1$ \cite{gao2017properties} and $\nabla^t$ is independent of $\bv^t$, we prove the following purely probabilistic result that will be used to bound the above summations to derive the final result.
    \begin{lemma} \label{lem:hoeff}
    Consider a set of vectors $\{y^1, ..., y^m\} \in [0,1]^n$ and let $\bY^1, ..., \bY^k$ be sampled without replacement from this set. Let $\bZ \in \ell_1^+$ be a random unit-vector that depends only on $\bY^1, ..., \bY^{k-1}$. Then for all $\ve > 0$,
    $$\Ex\langle \bY^k, \bZ \rangle \geq e^{-\ve} \min_i \{\Ex\bY^k_i\} - \frac{\ln n}{\ve \left(m - k + 1 \right)}.$$
    \end{lemma}
    %
    \eat{
    Intuitively, this lemma demonstrates the vitality of the reduction in correlation between items arriving in the online stream as a result of the restart in our algorithm. If, instead, $\bZ$ were highly dependent on $\bY^k$, in the worst case $\Ex \langle \bY^k, \bZ \rangle = \Ex \left[ \min_i \bY^k_i \right]$ which can be substantially greater than $\min_i \{\Ex \bY_i^k\}$.
    }
    %
    \begin{proof}
    Let $\mu = \frac{1}{m} \sum_t y^t$ be the average of the set of vectors and to simplify notation we additionally break apart the expectation and let $\Ex\langle \bY^k, \bZ \rangle = \Ex \left[ \Ex \left[ \langle \bY^k, \bZ \rangle | \bY^1, ..., \bY^{k-1} \right] \right]$. Note that since $\bZ$ is a unit-vector in $\ell_1^+$, an innerproduct of this vector with $\bY^k$ is simply a weighted sum of the latter's elements. Thus, we have
    \begin{align} \label{ineq.inner_prod}
        \Ex\left[ \langle \bY^k, Z \rangle | \bY^1, ..., \bY^{k-1} \right] %&=  \langle \Ex\left[\bY^k | \bY^1, ..., \bY^{k-1} \right], Z \rangle \\
        \geq \min_i \{ \Ex \left[ \bY^k | \bY^1, ..., \bY^{k-1}\right] \}.
    \end{align}
    Additionally, by nature of the sampling set and the procedure of sampling without replacement, we have the conditional expectation
    $$\Ex\left[ \bY^k | \bY^1, ..., \bY^{k-1} \right] = \frac{m\mu - (\bY^1 + ... + \bY^{k-1})}{m - (k - 1)}$$ and further note that $m\mu - (\bY^1 + ... + \bY^{k-1})$ has the \emph{same} distribution as $\bY^1 + ... + \bY^{m-(k-1)}$. This concretely gives us the simplifying equivalences
    $$\Ex\left[ \bY^k | \bY^1, ..., \bY^{k-1} \right] = \frac{m\mu - (\bY^1 + ... + \bY^{k-1})}{m-(k-1)} = \frac{\sum_{t=1}^{m-(k-1)} \bY^t}{m-(k-1)}.$$
    % and thus $\Ex\left[ \bY^k | \bY^1, ..., \bY^{k-1} \right]$ has the same distribution as $\frac{\bY^1 + ... \bY^{m-(k-1)}}{m - (k-1)}$. 
    %
    % Now taking expectations, we have
    %$$\Ex \left[ \min_i \{ \Ex\left[ \bY^k_i | \bY^1, ..., \bY^{k-1} \right] \} \right] = \frac{1}{m - (k - 1)}\Ex\left[ \min_i \{ \Ex\left[ \bY^1_i + ... + \bY^{m - (k - 1)}_i \right] \} \right]$$
    % Now noting that $\nabla^k \in \ell_1^+$ in Algorithm \ref{alg:smooth_greedy}, we can use Inequality (\ref{ineq:min_bound}) here and taking expectations we have
    % To bound this value, we invoke Inequality (\ref{ineq:min_bound}) and taking expectations we have
    % $$\sum_{t \leq k} \Ex \langle \bY^t, \bZ^t \rangle \leq e^\ve \left( \Ex \left[ \min_i \{ \sum_{t \leq k} \bY^t \}  \right] + \frac{\log n}{\ve}\right)$$
    We now return to the inequality bound of (\ref{ineq.inner_prod}) and, using the above equivalences, obtain 
    \begin{align*}
        \Ex \left[ \min_i \left\{ \sum_{t=1}^{m-(k-1)} \bY_i^t \right\} \right] &\geq \Ex \left[ \phi_\ve \left(\Sigma_{t=1}^{m-(k-1)} \bY^t \right) \right] \tag{Lemma \ref{lem:props}}\\
        &= \Ex \left[\frac{-1}{\ve} \ln \left( \sum_i \exp{\left(-\ve \Sigma_{t=1}^{m-(k-1)} \bY_i^t\right)} \right) \right]\\
        &\geq \frac{-1}{\ve} \ln \left( \sum_i \exp{\left(-\ve \Ex \left[ \Sigma_{t=1}^{m-(k-1)} \bY_i^t \right]\right)} \right) \tag{Jensen's Ineq.} \\
        &\geq e^{-\ve} \min_i \left\{ \Ex [\Sigma_{t=1}^{m-(k-1)} \bY_i^t] \right\} - \frac{\ln n}{\ve} \tag{Lemma \ref{lem:props}} \\
        &\geq e^{-\ve} \min_i \left\{ (m-(k-1)) \Ex \bY_i^t \right\} - \frac{\ln n}{\ve}
    \end{align*}
    %$$\Ex \left[ \min_i \{ \sum_{t=1}^{m-(k-1)} \bY^t \} \right] \geq e^{-\ve} \min_i \{ (m-(k-1)) \Ex \bY^t \} - \frac{\log n}{\ve}$$
    % \todo{cite this Chernoff result}
    
    \begin{comment}
    and since $\bZ^t$ is independent of $\bY^t$, we have $\Ex \langle \bY^t, \bZ^t \rangle = \langle \Ex \bY^t, \Ex\bZ^t \rangle.$ Thus, we can lower bound the left-hand side of the above inequality in the following manner:
    \begin{align*}
        \sum_{t \leq k} \Ex \langle \bY^t, \bZ^t \rangle &= \sum_{t \leq k} \langle \Ex \bY^t, \Ex \bZ^t  \rangle  \\
        &= \sum_{t \leq k} \langle \frac{\mu}{m} , \Ex \bZ^t \rangle \\
        &= \langle \mu, \frac{1}{m} \sum_{t \leq k} \bZ^t \rangle \\
        &\geq \min_i \{\mu_i\} \\
        &= \min_i \{\sum_{t \leq k} \Ex \bY^t\}
    \end{align*}
    where the inequality \todo{. . .}. Therefore, we have that $$\Ex \left[ \min_i \{ \sum_{t \leq m-(k-1)} \bY^t \}  \right] \geq e^{-\ve} \min_i \{\sum_{t \leq k} \Ex \bY^t\} - \frac{\ln n}{\ve}$$
\end{comment}
    
    \noindent %where the first and third inequalities come from Lemma \ref{lem:props}, and the second from repeated application of Jensen's inequality. 
    Finally combining the above results, we obtain
    \begin{align*}
        \frac{1}{m-(k-1)} \left(e^{-\ve} \min_i \{ (m-(k-1)) \Ex \bY^t \} - \frac{\ln n}{\ve} \right) &\leq \Ex \left[ \min_i \{\Ex \left[\bY^k_i | \bY^1, ..., \bY^{k-1} \right] \} \right] \\
        &\leq \Ex \langle \bY^t, \bZ \rangle
    \end{align*}
    Thus, after rearranging terms, this completes the lemma.
    \end{proof}
    
    \noindent Using this lower bounding result, we can now bound the sum of rewards as
    $$\Ex\left[ \langle \nabla^t, \bA^t\xopt^t \rangle \right] \geq e^{-\ve} \min_i \{\Ex\left[ \bA^t_i\xopt^t_i \right]\} - \frac{\ln n}{\ve(m - t + 1)}.$$
    Adding this result over all $t \leq \frac{m}{2}$ in combination with $\min_i \{\Ex\left[ \bA^t \xopt^t \right]_i\} = \frac{\opt{}}{m}$ we conclude that 
    \begin{align*}
        e^{2\ve} \cdot \Ex \sum_{t \leq \frac{m}{2}} \langle \nabla^t, \bA^t\bx^t \rangle &\geq \Ex \sum_{t \leq \frac{m}{2}} \langle \nabla^t, \bA^t\xopt^t \rangle \tag{Lemma \ref{lem:props}} \\
        &\geq e^{-\ve} \sum_{t \leq \frac{m}{2}} \min_i \{\Ex\left[ \bA^t_i\xopt^t_i \right]\} - \sum_{t \leq \frac{m}{2}} \frac{\ln n}{\ve(m - t + 1)} \\
        &= e^{-\ve} \left( \frac{\opt{}}{2}\right) - \frac{\ln n}{\ve}
    \end{align*}
    Due to the restart at $t = \frac{m}{2}$, we can extend the sum to $t = m$ by simply multiplying the above RHS by two. Finally, invoking inequality (\ref{ineq:min_bound}), we see that
    $$\Ex\left[ \min_i \bv^m \right] \geq e^{-4\ve} \opt{} - O \left(\frac{\log n}{\ve}\right) \geq \left(1-O(\ve)\right) \opt{} - O\left(\frac{\log n }{\ve}\right).$$
    by the Taylor approximation $e^{-x} \geq 1-x$ and the assumption on the size of \opt{}.\\ % \todo{randomized rounding of solution}
\end{proof}

==> prelim-scalar.tex <==
In this section, we introduce the notation that we will use in the rest of the paper. Let $\bv^1, ..., \bv^m \in [0,1]^n$ denote the input sequence of items arriving in random order where $v^t_i$ is the value of the $t$-th item to the $i$-th agent. We additionally denote by $\bx^1, ... , \bx^m \in [0,1]^n$ the fractional allocation of each item by the algorithm.
%
We further let the corresponding allocations of a fixed (offline) optimal solution be denoted as $\xopt^1, ..., \xopt^m \in [0,1]^n$ and let $\opt{}$ denote the max-min objective value of the optimal solution. 
%
For simplicity, we slightly abuse notation by letting $\bV^t = (v^t_1 x^t_1, \dots, v^t_n x^t_n)$ and $\bVo^t = (v^t_1 \overline{x}^t_1, \dots, v^t_n \overline{x}^t_n)$. Our algorithm thus seeks to maximize the coordinate-wise minimum of $\sum_{t=1}^m \bV^t$.
% \alert{I think the original matrix notation makes the analysis more readable but maybe less intuitive, working on better notation. The updated analysis and prelim are labeled -scalar.tex}
% Lastly, we define $\bv^t = \sum_{\tau=1}^t \bA^\tau \bx^\tau = (v_1^t, ..., v_n^t)$ be the vector of agent's allocation values up to time $t$. Our problem thus amounts to maximizing the component-wise minimum of $\bv^m$.
%$i$-th column of such a matrix which represents the value of item $j$ for agent $i$. Furthermore, this vector can only have a nonzero value in the $i$-th position: $\bA_{i}^j = (0,...,0,v_{ij},0,...,0)^T$. 
% We again note that in the random-order input model, an adversary selects the set $\{\bA^1, ..., \bA^m\}$ but the sequence {\em order} is random.
